Procedural Multiscale Geometry Modeling using Implicit Functions

Materials exhibit geometric structures across mesoscopic to microscopic scales, influencing macroscale properties such as appearance, mechanical strength, and thermal behavior. Capturing and modeling these multiscale structures is challenging but essential for computer graphics, engineering, and materials science. We present a framework inspired by hypertexture methods, using implicit functions and adaptive sphere tracing to synthesize multiscale structures on the fly without precomputation. This framework models volumetric materials with particulate, fibrous, porous, and laminar structures, allowing control over size, shape, density, distribution, and orientation. We enhance structural diversity by superimposing implicit periodic functions while improving computational efficiency. The framework also supports spatially varying particulate media, particle agglomeration, and piling on convex and concave structures, such as rock formations (mesoscale), without explicit simulation. We show its potential in the appearance modeling of volumetric materials and explore how spatially varying properties influence perceived macroscale appearance. Our framework enables seamless multiscale modeling, reconstructing procedural volumetric materials from image and signed distance field (SDF) synthetic exemplars using first-order and gradient-free optimization.

==> anisotropic.tex <==
\begin{figure*}
    \centering
    % First row of five main images with insets at the southeast corner
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_random_154_3.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/random_154.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_latticelike_154.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/clusters_lattice.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_pc_154_5.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/clustares_pc_154_5.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_pc_lattice10.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/clusters_lattice9.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_nc_154_3.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/regular_154.png}};
        \end{tikzpicture}
    \end{minipage}  \\ [-0.9ex]

     % Third row of five new main images with insets at the southeast corner
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f1-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_1.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f2-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_2.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f3-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_3.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f4-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_4.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f5-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_5.png}};
        \end{tikzpicture}
    \end{minipage} \\ [-0.9ex]

    % Second row of five main images with insets at the southeast corner
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_pc_clusters_154.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/fibers_clusters_154.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_pc_154_3_1.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/clusters_pc_154_1.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_pc_laminar3.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/fibers_clusters_laminar3.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_pc_154_3.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/clusters_154.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/fibers_pc_laminar2.png}};
            \node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/fibers_clusters_22.png}};
        \end{tikzpicture}
    \end{minipage} \\ [-0.9ex]
    
   

    % Fourth row of five new main images with insets at the southeast corner
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f6-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_6.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f7-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_7.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f8-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_8.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f9-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_9.png}};
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.19\linewidth}
        \begin{tikzpicture}
            \node[inner sep=0] (image) at (0,0) {\includegraphics[width=\linewidth]{images/f10-d.jpg}};
            %\node[anchor=south east, xshift=-0.1mm, yshift=-0.1mm] at (image.south east) {\includegraphics[width=0.3\linewidth]{images/inset_image_1.png}};
        \end{tikzpicture}
    \end{minipage}

    \caption{The first and third rows show the renderings of different anisotropic fibrous distributions obtained from polynomial functions using modular arithmetic on a regular spherical cloud. The different congruent classes for the modulo of the polynomial functions lead to different particle distributions, which can then stick to form the fibers. The density of fibers per cubic meter remains constant across all cases, but their distribution changes from left to right. Initially, the fibers are arranged loosely in clusters, and as we move toward the right, they transition into hard or sticky clusters from a random distribution. The individual fibers start to form tight clusters resembling laminar structures. The insets in the images illustrate their distribution, which varies from case to case. Additionally, the appearance of the fibrous material changes across the cases, and the difference images at the bottom for each case compared to the first leftmost case show how the arrangement of fibers within the volume leads to differences in appearance. }
    \label{fig:fiberclusters}
\end{figure*}



==> sections/intro.tex <==
\section{Introduction}



Real-world materials exhibit diverse microscopic structures that vary in shape, size, density, arrangement, and orientation. These geometric patterns are classified mainly into four categories: particulate, fibrous, laminar, and porous. Each category influences the properties and behaviors of the material. Understanding these classifications is essential for appearance modeling, engineering, biology, and material science applications.

Particulate materials consist of discrete particles that may be suspended, agglomerated, or in contact without merging. They vary in shape, density, arrangement, and size and can be crystalline or amorphous. Crystalline structures exhibit ordered, repetitive patterns, while amorphous structures lack periodicity and exhibit randomness \cite{zallen2008physics, callister2020materials}. Examples of particulate materials include ice, glass, diamonds, water, blood, and powders such as metal and sand. Some exist within a host medium, such as air bubbles in ice or red blood cells in plasma.


In appearance modeling, the translucency of a material is influenced by suspended particles that scatter light, shaping its visual properties~\cite{frisvad2007computing,jarabo2018radiative,guo2021beyond}. Although these optical properties enable realistic translucency effects, they limit the ability to closely examine individual particles. Multiscale modeling addresses this by preserving particle details~\cite{meng2015multi}. These particles add visual complexity at the mesoscopic scale, often lost in volume rendering but retained through detailed representation, enhancing realism.

To model particle-based materials, a common approach is to define a few particle types and arrange them within a tiled volume~\cite{meng2015multi}. However, tiling can introduce regularity issues and gaps due to density variations. To overcome this, we extend hypertexture methods with procedural modeling, simulating suspended particles, particle agglomerates, and particle piling without pre-generating them. Our method achieves high-density particulate materials without conventional volume rendering by computing the SDF for nearby particles.

Our approach allows control over particle shapes, sizes, and densities while enabling seamless zoom-in exploration. It also supports multi-scale density transitions within the same volume, ensuring smooth blending across scales, as demonstrated in Fig.\ref{fig:svbunny}. We focus on procedural tools for representing particles in a particulate medium rather than optimizing rendering efficiency. Modeling volumetric geometry is challenging, as a cubic centimeter contains nearly a trillion cubic microns, making explicit representation impractical due to memory constraints.

To overcome this, we introduce procedural methods for on-the-fly microgeometry generation, avoiding tiling subvolumes or scattering functions while leveraging existing rendering techniques~\cite{meng2015multi,muller2016efficient,michel2020real,zingsheim2024learning}. Our approach employs a 3D grid where cell indices seed a pseudo-random generator, enabling particle instantiation while ensuring controlled overlap within \(2^D\) nearest cells. Grid scaling, particle size, shape, and rejection sampling help achieve desired distributions. The dual grid approach only works for suspended particles and introduces artifacts for larger particles exceeding half the grid cell width. In such cases, particle agglomeration via SDF-based union operations requires evaluation across \(3^D\) nearest cells. Through particle agglomeration, particles can be joined based on algebraic functions to generate various other microstructures from the particles.


Various materials, such as ice, milk, cheese, metals, paper, and foams, present challenges due to their spatially varying geometries across different scales. Through particle agglomeration, we synthesize diverse microgeometries using a lattice of spherical particles inspired by blobby objects. While blobby object-based methods have been used for macro-level modeling~\cite{muraki1991volumetric,jin2005blob,kanamori2008gpu}, we extend this mechanism with hypertexture to generate volumetric microstructures efficiently. This approach allows for scalable modeling of fiber composites and other materials without expensive stochastic models~\cite{green2000stochastic}. By arranging spherical particles in a cubic grid and applying user-defined mod-$m$-polynomial functions, we achieve diverse microgeometries, see Fig.~\ref{fig:svbunny} for the visualization of the particle agglomeration, which is achieved using sampling particles based on polynomial functions applied to the suspended particulate media.



For granular media, such as rock piles and sand, we extend hypertexture models to procedurally generate rock piles on the fly, overcoming limitations of tiling-based methods~\cite{paris2020modeling,peytavie2009arches}. Our approach uses grid deformation with polynomial functions to model accurate contact positions while varying size, shape, and density; see Fig.~\ref{fig:svbunny}. One more advantage of our method is that we can generate grains that are concave in shape and their interactions on the fly. One important aspect is that we are not required to use collision detection methods to model the granular media.

Including spheres, our method supports all types of implicit primitives like cylinders, tubes, rings, and laminates, enabling realistic microstructure synthesis. Furthermore, we model microstructures using implicit periodic functions, specifically triply periodic minimal surfaces~\cite{han2018overview,dolan2015optical,inakage1987frequency,al2019multifunctional}. These sine and cosine-based structures create particulate, fibrous, laminar, and porous materials without discretizing grids, enabling fast evaluation and rendering. Both approaches grid-based and periodic functions offer trade-offs. The periodic approach enhances rendering speed, while the grid-based method provides greater spatial variation and multiscale microstructure synthesis.


Our contributions are procedural methods for modeling particulate, fibrous, laminar, and porous multiscale geometric patterns for modeling volumetric materials.
\begin{itemize}
\item Procedural modeling of multiscale geometric structures using SDFs in discrete grids and periodic functions for volumetric material synthesis.
\item We propose optimization-based reconstruction methods to reconstruct total volumetric SDFs from 2D slices of the volume containing SDFs.

\end{itemize}




==> supp_sections/future_work.tex <==
\section{Discussion and Future work}
There are several exciting future directions for this research. One potential avenue is to enhance the current framework by incorporating wave optics-based simulations to capture diffraction effects. Additionally, the inclusion of polarization and fluorescence could provide more depth to the analysis.

Another intriguing direction involves analyzing an input image of a particle cloud from a particular slice of a volume or a macroscopic rendering of the particulate material. In this case, we could extract particle size distributions and volume fractions to model the entire volume based on a specific patch or image of the material. This approach focuses on deriving particle statistics from the input data to reconstruct the complete volume. Techniques such as static light scattering, dynamic light scattering, or laser diffraction can be employed to measure these particle size distributions. Furthermore, neural network-based methods can aid in determining particle statistics from the available data on size distributions and volume fractions.

In this work, we focused solely on material appearance modeling utilizing multiscale geometry through SDFS. However, in the future, we plan to optimize various material properties, including thermal, mechanical, electrical, and chemical characteristics, in relation to the corresponding geometry at different length scales.

Another possible area of exploration is the generation of particle flow effects to simulate fluid motion, including the modeling of Brownian motion of particles.

% Reconstrution
In this paper, we explore some optimization strategies to reconstruct the geometric patterns from direct parameter fitting, image exemplars or incomplete volumetric information as a proof of concept with synthetic data. For future work, it would be interesting to reconstruct real microstructures using SEM/TEM images or microCT volumes. Reconstruction from SEM/TEM images would require to adapt the synthesis module to at least roughly mimic the appearance under an electronic microscope or ideally a suitable Monte Carlo simulator like Nebula. One possibility to handle the inability of our current reconstruction approaches to handle high-dimensional problems is to apply a surrogate loss~\cite{fischer2024zerograds} or explore neural network-based optimization techniques tailored for procedural models.   

% \subsection{Future Work}

% Finally, our inability to solve high-dimensional problems, highlights the need for more research into better global optimizers and improved loss function formulations. Potentially, next step could be to reformulate the problem as a simpler linear system of equations $\mathbf{Ax = b}$ and solve it using the recently developed learned preconditioning of the conjugate gradient~\cite{li2023learning}. Another promising direction could involve an iterative two-phase optimization approach: first, a 1D optimization of the noise-scale parameter, followed by optimizing the remaining parameters. This idea comes from the fact that the noise-scale influences every microstructure \ac{SDF} and has a significant impact on the visuals, often more so than the other parameters. 

% What's more, we find a big potential in the analysis-by-synthesis methods. However, the results show that the gradient-free optimization is not sufficient. Moving forward, we could either transform our pipeline to a differentiable one using for instance\cite{vicini2022differentiable, liu2020dist, jiang2020sdfdiff}, or potentially apply the surrogate loss using the ZeroGrads~\cite{fischer2024zerograds} on our analysis-by-synthesis loss.

% Furthermore, it would be worth exploring some \acp{INR}, such as the network with Gabor wavelet activation function~\cite{saragadam2023wire} or the \ac{MLP} with a trainable multiresolution hash encoding~\cite{muller2022instant}. A novel perspective on \acp{MLP} is offered by the \acp{KAN}~\cite{liu2024kan} which, according to the authors, should be superior to the tradional \ac{MLP} architecture. Another advantage of \acp{KAN} is their explainability, which allows the network to be reduced to an analytical formula. This could be a tool to discovering new \ac{SDF} representations of microstructures. An interesting direction of future research could also be to compare our \acp{INR} with the 1-Lipschitz Neural Distance Fields~\cite{coiffier20241}. 

% In addition, we believe that additional comparison metrics for microstructures could be introduced. The metrics we used tend to penalize small changes in linear transformations, which are unimportant in microstructure reconstruction. This is evident in the Figure~\ref{tab:comparison_contd}, in the example of the Gyroid[5D] when comparing CMA-ES-SDF and BH-SDF. One option is to fine-tune the \ac{LPIPS} network on the microstructure exemplars. 

% Finally, we would like to extend our microstructure dataset with real microstructures extracted from the \ac{microCT}. To obtain the signed distance fields from a real world CT scan, we could for instance adapt the technique introduced in \cite{park2019deepsdf}. To get the ground truth exemplar for the analysis-by-synthesis methods, any suitable render of the microstructure's \ac{microCT} scan image, where the patterns are clearly visible, can be used as the target, as long as the parameters $\mathbf{K}$ and $\mathbf{E}$ stay fixed and the shading somewhat corresponds to the \ac{BRDF} in the pipeline $\mathcal{R}$.


==> supp_sections/optimization.tex <==
\section{Multiscale Geometry Reconstruction}
\label{sec:optimization}

In this session, we address the reconstruction of the procedural microstructures introduced previously in session X with two approaches: parameter fitting and analysis by synthesis. The second approach leverages a rendering pipeline to guide the optimization, while the first one consists of a direct fitting of the procedural SDF. For each approach, we outline the optimization problem and its solution, including the required data, the loss functions, and optimization algorithms. To validate these approaches as a proof of concept, we focus on synthetic microstructures, assuming the availability of either a signed distance field or an RGB image.

% Juan Raul commets:
% (1) Diagram should be beautified or might entirely skipped
% (2) Too much detail for a session of a paper

\subsection{Parameter Fitting}
\label{parameter_fitting_approach}

This approach formulates microstructure reconstruction as a model-fitting task, where the goal is to optimize the parameters of a procedural SDF to accurately match the microstructure's SDF ground truth. Given a set of spatial coordinates $\Omega = \{\mathbf{x} \mid \mathbf{x} \in \mathbb{R}^3\}$, a ground-truth SDF $\hat{S}:~\mathbb{R}^3 \rightarrow \mathbb{R}$ describing the surface at point $x$, a bounded parameter space $\Phi = [a_1, b_1] \times [a_2, b_2] \times \cdots \times [a_n, b_n]$ with $n$ parameters, and a loss function $\mathcal{L}: \mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}$, the problem is defined as minimizing the discrepancy between the fitted function $f$ and the ground truth $\hat{S}$ across the domain: 
%
\begin{equation}
\min_{\boldsymbol{\phi} \in \Phi} \int_{\Omega} \mathcal{L}(f(\mathbf{x}, \boldsymbol{\phi}), \hat{S}(\mathbf{x})) d\mathbf{x}.
\end{equation}

$f$, in our case, is a suitable representation for the given microstructure. Procedural SDFs allow efficient extrapolation of the microstructure beyond the optimization domain without modifying the fitted function. In addition, our compact parametrized microstructures are described with a relatively low number of parameters. We propose a loss function to evaluate the discrepancies in the frequency domain using the discrete Fourier transform (DFT) to consider the periodic behavior common in many microstructures. The loss function compares the amplitude and phase spectra of the Fourier coefficients, using the logarithm of the mean squared error (MSE) as an error metric:
%
% \begin{multline}
% \mathcal{L}_{FT} \left( f(\Omega, \boldsymbol{\phi}), \hat{S}(\Omega) \right) =
% \log \biggl( \frac{1}{2N} \sum_{i=1}^{N} \Bigl( \left| A_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi}))) \\
% - A_i(\mathcal{F}(\hat{S}(\Omega))) \right|^2 + \left| \theta_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi}))) - \theta_i(\mathcal{F}(\hat{S}(\Omega))) \right|^2 \Bigr) + \epsilon \biggr),
% \label{FT_loss}
% \end{multline}

\begin{multline}
\mathcal{L}_{FT} \left( f(\Omega, \boldsymbol{\phi}), \hat{S}(\Omega) \right) = \\
\log \biggl( \frac{1}{2N} \sum_{i=1}^{N} \Bigl( \left| A_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi}))) - A_i(\mathcal{F}(\hat{S}(\Omega))) \right|^2 + \\
\left| \theta_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi}))) - \theta_i(\mathcal{F}(\hat{S}(\Omega))) \right|^2 + \epsilon \Bigr) \biggr).
\label{FT_loss}
\end{multline}

%
For simplicity we use $\Omega$ to express a series of points, $\mathcal{F}$ being a DFT,  $A_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi})))$ and $A_i(\mathcal{F}(\hat{S}(\Omega)))$ denoting the amplitudes, and \(\theta_i(f(\Omega, \boldsymbol{\phi}))\) and \(\theta_i(\hat{S}(\Omega))\) the phases of the Fourier coefficients derived from $f(\Omega, \boldsymbol{\phi})$ and $\hat{S}(\Omega)$, respectively, \(N\) representing the number of coefficients, and $\epsilon$ being a small positive value. Recall that $A_i(\mathcal{F}(x)) = |z_i| = \sqrt{\Re(z_i)^2 + \Im(z_i)^2}$, and $\theta_i(\mathcal{F}(x)) = \arctan\left(\frac{\Im(z_i)}{\Re(z_i)}\right)$, where $z_i$ is the $i$-th Fourier coefficient of $x$, and $\Re(z_i)$ and $\Im(z_i)$ are the real and imaginary parts of $z_i$, respectively. This loss is differentiable, enabling us to use gradient-based optimization algorithms as the operations involved are differentiable, including the DFT. Note this equation is closely related to the spectral density function commonly used in microstructure analysis~\cite{bostanabad2018computational}. 

For synthetic examples, ground-truth data generation consists of evaluating the corresponding target procedural SDF and its optimal parameters using a sampling method. Sampling points are generated within a transformed coordinate system as slices of a unit sphere in $\mathbb{R}^{D \times W \times H}$, aligned with the rotated basis vectors. These points are equidistant and centered at the origin, with Gaussian noise added to introduce small perturbations. Specifically, $i \in [1, D]$, $j \in [1, W]$, and $k \in [1, H]$ represent the indices corresponding to the generated points in the respective directions, and $\bar{\mathbf{x}}$ is a point inside the coordinates space with standard basis:

\begin{equation}
    \Omega = \left\{ \bar{\mathbf{x}}_{i,j,k} + \boldsymbol{\epsilon}_{i,j,k} \mid \boldsymbol{\epsilon}_{i,j,k} \sim \mathcal{N}(0, \sigma^2 \mathbf{I}) \right\}. 
\end{equation}
\label{point_generation_equation} 

Selecting a suitable optimization algorithm is critical for solving unconstraint global optimization problems. We employ two first-orded methods taking advantage of the gradient information: Basin-Hoppin(BH)~\cite{wales2003energy} and Simplicial Homology Global Optimization (SHGO)\cite{endres2018simplicial} algorithms. The BH algorithm is particularly effective for problems with funnel-like loss functions. Its key hyperparameters include the step size $s$ and the temperature $T$, which define the bounds of the uniformly distributed random perturbations and the acceptance probability for the candidate function, respectively. The temperature $T$ is empirically set to $T = 0.001$. Additionally, the Sequential Least-Squares Quadratic Programming (SLSQP) algorithm is used as a local minimizer in the second phase, which iteratively solves a QP subproblem derived from a second-order Taylor expansion of the loss function. The BH algorithm requires an initial $\boldsymbol{\phi}_0$. SHGO global optimization algorithm approximates locally convex subdomains using homology groups. The main hyperparameters for SHGO include the number of iterations  $l$ and the number of samples  $m$ for building the complex. Depending on problem complexity, we typically select $m \in [10,10000]  \cap \mathbb{N}$ and set $l = 1$. The Sobol sampling method and SLSQP are used for local search. Unlike the BH algorithm, SHGO does not require an initial population mean $\boldsymbol{\phi}_0$ but requires variable bounds.

As previously noted, the loss function is differentiable, but certain procedural SDFs are not differentiable, leading to non-differentiability of the final composite function $\mathcal{L} \circ f$. For gradient-free cases, we use the Covariance Matrix Adaptation Evolutionary Strategy (CMA-ES) algorithm~\cite{hansen2019pycma} as it is highly effective, in particular for rugged and non-differentiable problems. Its key hyperparameters are the population size $\mathcal{P}$ and the initial $\sigma_0$ of the covariance matrix, typically chosen depending on the complexity and dimensional of the problem. In our case, $\mathcal{P} \in [40, 400]$ and $\sigma_0 \in [70, 250]$. CMA-ES requires an initial population mean $\boldsymbol{\phi}_0$. 

\subsection{Analysis by Synthesis}
\label{analysis_by_synthesis_approach}

The main difference between the analytical optimization-based approach discussed in the first section and the analysis-by-synthesis method lies in the comparison process. Despite this difference, both methods aim to find an optimal SDF. In the latter approach, we employ a non-differentiable rendering pipeline to visualize the SDF and subsequently compare the resulting renders. Given a camera intrinsics $\mathbf{K} \in \mathbb{R}^{3\times 3}$ taken from a set of intrinsic matrices $\mathcal{K}$, the camera extrinsics $\mathbf{E} = [\mathbf{R} \mid \mathbf{t}] \in \mathbb{R}^{3\times 4}$  taken from a set of extrinsic matrices $\mathcal{E}$, a labeling function $\hat{S}:~\mathbb{R}^3 \rightarrow \mathbb{R}$, a bounded parameter space $\Phi = [a_1, b_1] \times [a_2, b_2] \times \cdots \times [a_n, b_n]$ with $n$ parameters, a signed distance fitting function $f: \mathbb{R}^3 \times \Phi \rightarrow \mathbb{R}$, a loss function $\mathcal{L}: \mathbb{R}^{W\times H \times 3} \times \mathbb{R}^{W\times H \times 3} \rightarrow \mathbb{R}$, with $W, H$ being width and the height respectively, a set of functions $\mathcal{A}$, and finally the rendering function $\mathcal{R}:~\mathcal{A}\times \mathcal{K} \times \mathcal{E} \rightarrow \mathbb{R}^{W\times H \times 3}$, we can express the problem as follows:

\begin{equation}
    \min_{\boldsymbol{\phi} \in \Phi} \mathcal{L}\left( \mathcal{R}\left( f\left( \cdot, \boldsymbol{\phi}\right), \mathbf{K}, \mathbf{E}\right), \mathcal{R} ( \hat{S}\left( \cdot \right), \mathbf{K}, \mathbf{E} ) \right).
\label{analysis_by_synthesis_eq}
\end{equation}

$\mathcal{R}$ renders the microstructure bounded by a unit sphere from the given view with the camera parameters using the sphere-tracing algorithm~\cite{hart1996sphere} in the CUDA-based framework OptiX \cite{parker2010optix}. Similar to the parameter fitting approach, we can set $f := \hat{f}$. To generate the ground-truth data for the analysis-by-synthesis approach, we must provide a target render image. This involves rendering the microstructure using the $\mathcal{R}\Bigl(\hat{S}(\cdot), \mathbf{K}, \mathbf{E} \Bigr)$ with a fixed $\mathbf{K}, \mathbf{E}$ later used for the optimization.\\ 

For the loss function, we use the two-dimensional DFT, denoted as $\mathcal{F}_{2D}$, to transform the image signal for comparison in the frequency domain expressed as:
%
% \begin{multline} \mathcal{L}_{2DFT} \left( \mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E}), \mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E}) \right) = \\
% \log \biggl( \frac{1}{N} \sum_{i=1}^{N} \left| A_i\Bigl(\mathcal{F}_{2D}(\mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E})) \Bigr) - \\ 
% A_i \Bigl(\mathcal{F}_{2D}(\mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E})) \Bigr) \right|^2 + \epsilon \biggr), 
% \label{FT_loss_image}
% \end{multline}
%
\begin{align}
\mathcal{L}_{2DFT} &\left( \mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E}), \mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E}) \right) = \notag \\
&\log \biggl( \frac{1}{N} \sum_{i=1}^{N} \left| A_i\Bigl(\mathcal{F}_{2D}(\mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E})) \Bigr) - \right. \notag \\
&\quad \left. A_i \Bigl(\mathcal{F}_{2D}(\mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E})) \Bigr) \right|^2 + \epsilon \biggr),  
\label{FT_loss_image}
\end{align}



where $A_i\Bigl(\mathcal{F}_{2D}(\mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E}))\Bigr) $ and $A_i\Bigl(\mathcal{F}_{2D} (\mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E}) ) \Bigr)$ denote the amplitudes of the 2D Fourier coefficients for the rendered image and the target image, respectively. $N$ represents the total number of coefficients, and $\epsilon$ is a small constant. By focusing on the amplitudes of the Fourier coefficients, we capture the key periodic features of the image, which proved to be crucial for effective global optimization in our experiments. While multi-view optimization is theoretically possible, we opted for single-view optimization due to its computational overhead, as rendering multiple views would be even more time-consuming.\\ 

In this approach, the rendering function $\mathcal{R}$ is non-differentiable, forcing us to only use gradient-free optimizers. The first optimizer we consider is again the evolutionary algorithm CMA-ES \cite{hansen2019pycma} as it is gradient-free, adaptive, robust to noise, and effective in complex landscapes. As the evaluation of the loss function in Equation~\ref{FT_loss_image} is computationally expensive due to the overhead of $\mathcal{R}$, we decide to decrease the population size to $\mathcal{P} \in [5, 10] \cap \mathbb{N}$. For our microstructure experiments, we maintain the initial standard deviation at $\sigma_0 \in~[60, 80]$. The second optimization algorithm that we considered is the slightly modified Powell method \cite{press1988numerical, powell1964efficient}, a local optimizer without hyperparameters that can be proven to be effective when a reasonable close initialization is provided. 

% \subsection{Implementation Details}
% \label{implementation_details}

% The microstructure is rendered in white, with a basic Lambertian reflection model applied as our simple BRDF. We found $W = 400, H = 400$ to be sufficient for the optimization. For a better visualization, we include a background image.

% We use the SciPy \cite{2020SciPy-NMeth} implementation of the \ac{BH}, \ac{SHGO} and the Powell method. We use the \ac{CMA-ES} \cite{hansen2019pycma} implementation. We use the PyTorch's auto-differentiation $\cite{paszke2017automatic}$ functionality for obtaining gradients when possible and appropriate. 

% To visualize the fitted microstructure given by $f(\cdot, \boldsymbol{\phi}^*)$, found by Approaches~\ref{Analytical_sdf_based_approach} and \ref{analysis_by_synthesis_approach}, we use the OptiX ray-tracing framework~\cite{parker2010optix}, before denoted as $\mathcal{R}$. OptiX is a recursive rendering pipeline with flexible shader composition. Simply put, the framework generates rays from the camera pinhole in a manner defined by the user. The rays then traverse through the scene until a miss or closest hit shader is invoked. In the case of a miss, the framework returns the environment map's color. When a geometry hit is detected (with our scene consisting only a unit sphere), we employ a sphere-tracing algorithm. This algorithm either returns the shaded microgeometry within the unit sphere using the Lambertian reflection model or continues traversing until it returns the environment map color. The lifecycle of OptiX is illustrated in the.

% The sphere tracing algorithm queries the distance function $f$. This requires two main tasks: 1. loading the optimal parameters $\boldsymbol{\phi}^*$ to the GPU, and 2.~implementing the function $f$ within a CUDA shader.

% To load the $\boldsymbol{\phi}^*$ or $\boldsymbol{\theta}^*$, we save the optimal parameters into a NumPy \cite{harris2020array} array. This array is then loaded within the C++ code using the libnpy library~\cite{libnpy} and uploaded to the GPU before ray generation. We use this procedure for both the function parameters found by the Approaches~\ref{Analytical_sdf_based_approach},~\ref{analysis_by_synthesis_approach}.  Rendering pipeline parameters, such as the $\mathbf{K}, \mathbf{E}$ and the reference to the NumPy array with parameters, are stored inside a JSON file and passed as an argument to the C++ code.

% To query $f$, we implement the function in the CUDA shader. We use our own implementation of the microstructure fitting functions $\hat{f}$. A minor drawback of this approach is the need to implement the $f$ in both CUDA and the PyTorch framework for the Approach~\ref{Analytical_sdf_based_approach}. For the Approach~\ref{analysis_by_synthesis_approach}, the CUDA implementation is sufficient. The full code is available in the supplementary material provided with the thesis and can also be accessed on the private GitHub repository upon request~\cite{my_repo}.

% \section{Results and analysis}

% In this chapter, we demonstrate the results of our experiments. The results section is divided into the following parts: First, we introduce the synthetic dataset used to evaluate our methods. Next, we showcase the outcomes of the experiments, followed by a discussion of the findings and possible areas for improvement.

% To ensure reproducibility, we provide the code with the paper. In addition to that, we have prepared a Jupyter Notebook script which can reproduce all of the results presented in this chapter: \texttt{optimization\_reconstruction.ipynb}, which covers the analytical optimization-based approach (described in the Section \ref{Analytical_sdf_based_approach}) and the analysis-by-synthesis method (covered in the Section \ref{analysis_by_synthesis_approach}).

% \subsection{Synthetic Dataset}
% \label{synthetic_dataset}

% \begin{figure}[ht]
%     \centering
%     \begin{adjustbox}{max width=\textwidth, max height=0.17\textheight}
%     \setlength{\tabcolsep}{7.7pt} % Adjust column separation
%     \renewcommand{\arraystretch}{0.3} % Adjust row separation
%     \begin{tabular}{c c c}
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-0_resized.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-1.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-2.png}\\
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-3.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-4.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-5.png} 
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Instances of exemplar renders (\textit{top row}) Gyroid~[1D], Fibers~[2D], Gyroid~[3D] respectively. Rest of the renders (\textit{bottom row}) are Spheres~[2D], Gyroid~[5D], Porous~[28D] respectively.}
%     \label{tab:renders_exemplars}
% \end{figure}

% For the proof of concept and more control over the experiments, we test our algorithms on representative synthetic examples that closely resemble \ac{SEM}/\ac{TEM} images. The dataset consists of six microstructures. Each microstructure is defined by a \ac{SDF} $\hat{f}$ with $n$ parameters, denoted as $\boldsymbol{\phi}$ in Approaches~\ref{Analytical_sdf_based_approach} and~\ref{analysis_by_synthesis_approach}. We include the number of parameters inside square brackets in the naming conventions to reflect both the degrees of freedom and to provide an indication of the optimization complexity. The renders of the exemplars can be seen in the Figure~\ref{tab:renders_exemplars}. All ground-truth parameter values presented in the dataset were selected for their convenience and to ensure they fit in the defined domain range.

% \subsection{Set-Up}

% To set up the analytical optimization-based approach (see Section~\ref{Analytical_sdf_based_approach}), we generate a set of points $\Omega$ on a discrete grid, with dimensionality ranging from $400 \times 400 \times 10$ (approximately 800,000 points) for lower-dimensional problems, up to $400 \times 400 \times 41$ (about 6.5 million points) for higher-dimensional cases. The optimizer hyperparameter values align with the intervals specified in the Section~\ref{optimization_analytical_approach}. To ensure a fair comparison between the optimization algorithms used in this approach, the same data is used across all methods.

% For the set-up of the analysis-by-synthesis methods, we fix the camera intrinsics~$\mathbf{K} \in \mathbb{R}^{3\times 3} $ and the camera extrinsics $[\mathbf{R} \mid \mathbf{t}] \in \mathbb{R}^{3\times 4}$ for each microgeometry. It is worth noting that the $\mathbf{K}$ is simplified, with the only parameter being the focal length (or field of view), while the other parameters are fixed on standard assumptions, e.g. zero skew and optical center at the image midpoint. Using such a setup and the mentioned sphere tracing framework, we render the ground truth image $\mathcal{I} \in \mathbb{R}^{W\times H \times 3}$. For all optimizations, we fix $W=400, H=400$. To ensure a fair comparison, the same ground truth image is used across all optimizers in the approach.

% Additionally, we generate a validation dataset $\Omega_\text{val}$ consisting of a grid of around 1 million points to validate the generalizability. 

% The hyperparameters of each method are adjusted for the specific microstructure. Initial values  and variable bounds are set uniformly across all optimizers to ensure meaningful comparisons. These values were determined through a process of trial and error of visualizing the microstructure with different parameter values. Initial values for each microstructure can be found in the code. For more details about the hyperparameters of all approaches, please see the Jupyter Notebook \texttt{optimization\_reconstruction.ipynb}.

% We conducted all of the experiments for Approaches~\ref{Analytical_sdf_based_approach} and \ref{analysis_by_synthesis_approach} on a personal laptop equipped with a GeForce RTX 4060 GPU (8GB VRAM), 16GB RAM, and an Intel i7-13620H processor.

% \subsection{Optimization Results}

% The comparison of the the function fitting global optimizers used for methods~\ref{Analytical_sdf_based_approach}, \ref{analysis_by_synthesis_approach} evaluated on our synthetic dataset (Section~\ref{synthetic_dataset}), can be observed in the Table~\ref{optimization_table_results} below. For each of the microgeometry in the row, we 
% list the following measured indications: \textbf{a)} Validation error computed as a sum of MAE of signed distances and error in the cosine similarity of gradients: 
% \begin{multline}
% \label{validation_error}
% \text{Val. Error} = \frac{1}{|\Omega_{\text{val}}|} \sum_{\mathbf{x} \in \Omega_{\text{val}}} \left| f(\mathbf{x}, \boldsymbol{\phi}) - \hat{S}(\mathbf{x}) \right| \\
% + \frac{1}{|\Omega_{\text{val}}|} \sum_{\mathbf{x} \in \Omega_{\text{val}}} \left( 1 - \frac{\nabla f(\mathbf{x}, \boldsymbol{\phi})^T \nabla \hat{S}(\mathbf{x})}{\|\nabla f(\mathbf{x}, \boldsymbol{\phi})\| \|\nabla \hat{S}(\mathbf{x})\|} \right),
% \end{multline}

% where $\Omega_{\text{val}}$ is the validation dataset, and $\boldsymbol{\phi}$ are the found parameters, otherwise the notation follows the Chapter \ref{methods_chapter}. We also present \textbf{b)}~Perceptual loss of the rendered solution and the ground truth image using the VGG-based network of the \ac{LPIPS} \cite{perceptual_loss, simonyan2014very}. It is important to note that the \ac{LPIPS} (as specified by the authors) was trained on 161k distorted patches extracted from the MIT-Adobe 5k dataset \cite{fivek} which includes photographs taken in the wild. This is by no means similar to the microstructure images we are dealing with, nevertheless, we find the loss to be quite meaningful, as we show later. Furthermore, we also present \textbf{c)} Low dynamic range image \FLIP error of the rendered solution and the ground truth render \cite{andersson2020flip}, \textbf{d)}~Time of the optimization and
% \textbf{e)}~The difference between the loss at the beginning and at the end of the optimization process denoted as $\Delta$-loss which gives the reader an idea of how much the loss improves. We do not list in the table the minimum loss reached per optimizer due to the inconsistency of the used losses per scenario.

% The time limit for all examples was set to 20~minutes, as results typically do not improve significantly beyond this point. We consider a numerical~0 to be a number below $1\times10^{-7}$. We denote the analytical optimization-based function fitting using the "SDF" suffix and the analysis-by-synthesis function fitting by the "S" suffix in the names of the methods in the Table~\ref{optimization_table_results}. The best results are highlighted in orange, while the second-best results are marked in yellow. Note that both \ac{SHGO} and \ac{BH} optimizers are in some cases not applicable, as they require differentiability, which is not a property of the Spheres~[2D]. Moreover, the preprocessing of \ac{SHGO} takes too long for the Porous~[28D] example, preventing it from producing any meaningful results within the 20-minute limit.

% \begin{table}[ht]
% \begin{adjustbox}{max width=\textwidth, max height=0.2\textheight, center}
% \begin{tabular}{l r | >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm}} 
% Microstructure & & SHGO-SDF & BH-SDF & CMA-ES-SDF & CMA-ES-S & Powell-S\\
% \toprule
%     % \multirow{5}{*}{Gyroid [1D]} & MAPE$\downarrow$ & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$\% & \cellcolor{orange!25}$\mathbf{1\times10^{-3}\%}$ & \cellcolor{orange!25}$\mathbf{4\times10^{-2}}\%$ & 14.6\% & 0.53\%\\ 
%     \multirow{5}{*}{Gyroid [1D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & $10^{-4}$ & \cellcolor{yellow!25}$10^{-6}$\\ 
% & LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{orange!25}\textbf{0.00}& \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.02 & \cellcolor{orange!25}\textbf{0.00}\\ 
% & \FLIP$\downarrow$ &  \cellcolor{yellow!25}$3\times10^{-7}$  & \cellcolor{orange!25}$\mathbf{1\times10^{-7}}$ &  $1\times10^{-3}$  &  $2\times10^{-3}$ &  $2\times10^{-3}$\\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{2.85s}  & \cellcolor{yellow!25}16.67s & \cellcolor{orange!25}\textbf{2.23s}  & 20m & 7m\\ 
% & $\Delta$-loss$\uparrow$ & 23.67 & 23.87 & 19.25  & 4.55 & 8.12 \\
% \\
% % \multirow{5}{*}{Fibers [2D]} & MAPE$\downarrow$ & 106.03\% & \cellcolor{orange!25}\textbf{2.55}\% & 487.82\% & 693.64\% & 806.59 \%\\ 
% \multirow{5}{*}{Fibers [2D]} & Val. Error$\downarrow$ & \cellcolor{yellow!25}0.34 & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & 0.65 & 1.00 & 1.00\\ 
% & LPIPS$\downarrow$ & \cellcolor{yellow!25}0.41 & \cellcolor{orange!25}\textbf{0.13} & 0.54 & 0.56 & 0.56   \\ 
% & \FLIP$\downarrow$ &  \cellcolor{yellow!25}0.3  & \cellcolor{orange!25}\textbf{0.14} & 0.42  &  0.40 &  0.43 \\ 
% & Time$\downarrow$ & 13m  & 20m & \cellcolor{yellow!25}6m  & 20m & \cellcolor{orange!25}\textbf{5m}\\ 
% & $\Delta$-loss$\uparrow$   & 2.17 & 7.58 & 1.46  & 0.08 & 0.05 \\ 
% \\
% % \multirow{5}{*}{Gyroid [3D]} & MAPE$\downarrow$ & 0.07\% & \cellcolor{orange!25}\textbf{0.01\%} & 1893.16\%& 346.27\% & 7.46\%\\ 
% \multirow{5}{*}{Gyroid [3D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & $6\times10^{-3}$ & 1.02& 0.15 & \cellcolor{yellow!25}$2\times10^{-3}$\\ 
% & LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.01} & 0.04 & 0.65 & 0.35 & \cellcolor{yellow!25}0.02\\ 
% & \FLIP$\downarrow$ &  \cellcolor{orange!25}\textbf{0.01}  & 0.05 &  0.61 &  0.42 &  \cellcolor{yellow!25}0.03 \\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{22.7s} & 20m & \cellcolor{yellow!25}7m & 14m & 20m\\ 
% & $\Delta$-loss$\uparrow$   & 18.2 & 18.88 & 0.72& 1.64 & 4.66 \\ 
% \\
% \multirow{5}{*}{Spheres [2D]} & Val. Error$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}$\mathbf{1\times10^{-5}}$ & 1.01 & 1.01\\ 
% & LPIPS$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{0.00} & 0.53 & 0.53\\ 
% & \FLIP$\downarrow$ &  \sout{N/A}& \sout{N/A} & \cellcolor{orange!25}$\mathbf{3\times10^{-7}}$  &  0.55 & 0.55 \\ 
% & time$\downarrow$ &\sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{4m}  & 20m & 5m\\ 
% & $\epsilon$-loss$\uparrow$  & \sout{N/A} &\sout{N/A} & 11.34  & 0.63 & 0.61 \\ 
% \\
% \multirow{5}{*}{Gyroid [5D]} & Val. Error$\downarrow$ & 0.66 & 0.65 & \cellcolor{orange!25}\textbf{$\mathbf{3\times10^{-4}}$} & \cellcolor{yellow!25}0.03 & 0.44 \\ 
% & LPIPS$\downarrow$ & 0.42 & 0.57 & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.21 & 0.54 \\ 
% & \FLIP$\downarrow$ &  0.42  & 0.62 &  \cellcolor{orange!25}\textbf{$\mathbf{6\times10^{-3}}$}  &  \cellcolor{yellow!25}0.28 &  0.60\\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{2m} & 15m & \cellcolor{yellow!25}11m  & 20m & 15m \\ 
% & $\Delta$-loss$\uparrow$  & 1.92 & 1.75 & 20.34  & 2.14 & 1.60\\ 
% \\
% \multirow{5}{*}{Porous [28D]} & Val. Error$\downarrow$ & \sout{N/A} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00}\\ 
% & LPIPS$\downarrow$ & \sout{N/A} & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{orange!25}\textbf{0.61}\\ 
% & \FLIP$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{0.51} & \cellcolor{yellow!25}0.52 & \cellcolor{yellow!25}0.52 & 0.59\\ 
% & Time$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{4m} & \cellcolor{yellow!25}8m & 20m & 20m\\ 
% & $\Delta$-loss$\uparrow$  & \sout{N/A} & 0.88 & 0.01 & 1.6 & 0.23\\ 
% \end{tabular}
% \end{adjustbox}
% \caption{Fitted Functions. Table of comparison of the global optimization algorithms used on our sythetic dataset~\ref{synthetic_dataset}. We show for each problem the following: \textbf{a)} Validaton Error~\ref{validation_error}, \textbf{b)} LPIPS Perceptual loss, \textbf{c)} \FLIP error, \textbf{d)} Time of the optimization, \textbf{e)} The difference between the loss at the beginning and at the end of the optimization process denoted as $\Delta$-loss. The time limit for all examples was set to 20~minutes. We consider a numerical~0 to be a number below $1\times10^{-7}$. The \sout{N/A} implies that the method could not be used for the problem. }
% \label{optimization_table_results}
% \end{table}

% To show the full story behind the optimization process, we present the plot depicting the log loss as a function of iteration in the Figure~\ref{fig:plot_losses_optmimization} of the Gyroid~[5D] and Fibers~[2D] microstructures. Plots of the rest microstructure optimizations can be found in the Appendix~\ref{tab:plots_losses_optimization_based_appendix}.

% \begin{figure}[ht!]
%     \centering
%     \begin{adjustbox}{max width=1.0\textwidth, max height=1.0\textheight, keepaspectratio}
%     \renewcommand{\arraystretch}{1.5} % Adjust row height
%     \setlength{\tabcolsep}{2pt} % Adjust column spacing
%     \begin{tabular}{c c}
%         \includegraphics[width=1.0\linewidth]{figures/plots/losses_gyroid_5D.png} & 
%                 \includegraphics[width=1.0\linewidth]{figures/plots/losses_two_variable_fiber.png}   
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Function Fitting. Function $\log_{10}$ loss of iteration of a Gyroid~[5D]~(\textit{left column}) and Fibers~[2D] (\textit{right column}) microstructure. The first (\textit{top row}) subplots show losses of the analytical optimization-based methods~\ref{FT_loss}. The second (\textit{bottom row}) subplots show losses of analysis-by-synthesis methods~\ref{FT_loss_image}. The best-reported solution by the optimizer is marked using a diamond marker.}
%     \label{fig:plot_losses_optmimization}
% \end{figure}

% For each microstructure optimization plot, the top row displays the loss for analytical optimization-based methods (Section~\ref{FT_loss}), while the bottom row illustrates the loss for analysis-by-synthesis methods (Section~\ref{FT_loss_image}). The best-reported solution by the optimizer is marked using a diamond marker. Each loss function was smoothed using a smoothing window of size~5. We follow the same naming convention from the Table~\ref{optimization_table_results}.

% Finally, we present the comparisons of rendered ground truth exemplars and the rendered fitted approximations in the Figures~\ref{tab:comparison}, \ref{tab:comparison_contd}. 
% Per each microstructure of the synthetic dataset (Section~\ref{synthetic_dataset}), we show the rendered reference (\textit{outermost left column}), two (one for the Spheres [2D]) best analytical optimization-based method(s) (\textit{left column(s)}), the best (two best for the Spheres [2D]) analysis-by-synthesis method(s) (\textit{right column(s)}). The best methods in each section are selected based on the validation error \ref{validation_error}.  We describe in the title the name of the method together with the validation error in the brackets, also specified in the Table~\ref{optimization_table_results}, while following its naming convention. 

% \definecolor{darkorange}{RGB}{255,140,0}  % RGB values for dark orange
% \begin{figure}[ht!]
%     \begin{adjustbox}{max width=\textwidth, max height=0.5\textheight}
%     \setlength{\tabcolsep}{5.7pt} % Adjust column separation
%     \renewcommand{\arraystretch}{1.3} % Adjust row separation
%     \arrayrulecolor{darkorange}
%     \setlength{\dashlinedash}{4pt} % length of dashes
%     \setlength{\dashlinegap}{4pt}  % gap between dashes
%     \setlength{\arrayrulewidth}{0.45mm} % thickness of the lines
%     \begin{tabular}{c c : c @{\hspace{0.1cm}} c : c}
    
%         & Reference & BH-SDF ($0.00$) & SHGO-SDF ($0.00$) & Powell ($10^{-6}$)\\ 
%         \multirow{2}{*}{\rotatebox{90}{\centering Gyroid [1D]}} & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-0_resized.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_0_resized.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-SHGO_0_resized.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-Powell-S_0.png}
%         \\
%         & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_0.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/SHGO_0.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/gyroid1d_siren_volume_256.png}
%         \\
        
%         &  & BH-SDF ($10^{-3}$) &  SHGO-SDF (0.34) & CMA-ES-S (1.00) \\ 
%         \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{Fibers [2D]}}} & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-1_resized.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_1_resized.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-SHGO_1_resized.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_1.png}
%          \\ 
%         & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_1.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/SHGO_1.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_1.png}
%         \\
         
%         &  & SHGO-SDF ($10^{-3}$) & BH-SDF ($6\times10^{-3}$) & Powell-S ($2\times10^{-3}$) \\ 
%         \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{ Gyroid [3D]}}} & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-2_resized.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-SHGO_2_resized.png} &
%                 \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_2_resized.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-Powell-S_2.png} 
%          \\ 
%         & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/SHGO_2.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_2.png} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/Powell-S_2.png}  
%         \\
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Renders Comparisons (\textit{continued in the next figure}). Comparison of rendered ground truth exemplars and the rendered approximations~(\textit{top row per microstructure}) with the measured \FLIP (\textit{bottom row per microstructure}). \textit{Outermost left column:}~Rendered reference. \textit{Two left columns:}~Two best analytical optimization-based methods. \textit{Right column:}~The best analysis-by-synthesis method. The best methods in each section are selected based on the validation error \ref{validation_error}.  We describe in the title the name of the method together with the val. error in the brackets, also specified in the Tables~\ref{optimization_table_results}. }
%     \label{tab:comparison}
% \end{figure}

% \begin{figure}[ht!]
%     \begin{adjustbox}{max width=\textwidth, max height=\textheight}
%     \setlength{\tabcolsep}{5.7pt} % Adjust column separation
%     \renewcommand{\arraystretch}{1.3} % Adjust row separation
%     \arrayrulecolor{darkorange}
%     \setlength{\dashlinedash}{4pt} % length of dashes
%     \setlength{\dashlinegap}{4pt}  % gap between dashes
%     \setlength{\arrayrulewidth}{0.45mm} % thickness of the lines
%     \begin{tabular}{c c : c c : c}
        
%        & Reference & CMA-ES-SDF ($10^{-5}$) & \multicolumn{1}{:c@{\hspace{-0.1cm}}}{CMA-ES-S (1.01)} & Powell-S (1.01)) \\ 
%         \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{ Spheres [2D]}}} & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-3_resized.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES_3_resized.png} &
%         \multicolumn{1}{:c@{\hspace{-0.1cm}}}{\includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_3.png}} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-Powell-S_3.png}
%          \\ 
%         & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_3.png} &
%         \multicolumn{1}{:c@{\hspace{-0.1cm}}}{\includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_3.png}} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/Powell-S_3.png}
%         \\
%          \cdashline{4-4}
%         &  & CMA-ES-SDF ($3\times10^{-4}$) & \multicolumn{1}{@{\hspace{-0.2cm}}c:}{BH-SDF(0.65)} & CMA-ES-S (0.03) \\ 
%         \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{ Gyroid [5D]}}} & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-4_resized.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES_4_resized.png} &
%         \multicolumn{1}{@{\hspace{-0.2cm}}c:}{\includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_4.png}} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES_4_resized.png}
%          \\ 
%          & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_4.png} &
%         \multicolumn{1}{@{\hspace{-0.2cm}}c:}{\includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_4.png}} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_4.png}
%         \\
%         &  & BH-SDF ($1.00$) & \multicolumn{1}{@{\hspace{-0.2cm}}c:}{CMA-ES-SDF(1.00)} & CMA-ES-S (1.00) \\ 
%         \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{ Porous [28D]}}} & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-5.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render_5_BH.png} &
%         \multicolumn{1}{@{\hspace{-0.2cm}}c:}{\includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render_5_CMA_ES.png}} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render_5_CMA_ES_S.png}
%          \\ 
%          & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_BH.png} &
%         \multicolumn{1}{@{\hspace{-0.2cm}}c:}{\includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_CMA_ES.png}} &
%         \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_CMA_ES_S.png}
%         \\
%     \end{tabular}
%     \end{adjustbox}
%     \caption{Renders Comparisons (\textit{continuation}). Comparison of rendered ground truth exemplars and the rendered approximations~(\textit{top row per microstructure}) with the measured \FLIP (\textit{bottom row per microstructure}). \textit{Outermost left column:}~Rendered reference. \textit{Two~(one for Spheres [2D])~left column(s):}~Two best analytical optimization-based methods. \textit{Right (two for Spheres [2D]) column(s):}~The best analysis-by-synthesis method(s). The best methods in each section are selected based on the validation error \ref{validation_error}.  We describe in the title the name of the method together with the val. error in the brackets, also specified in the Tables~\ref{optimization_table_results}. }
%     \label{tab:comparison_contd}
% \end{figure}

% \subsection{Discussion}

% Let us compare respectively the analytical optimization-based methods and the analysis-by-synthesis methods. We conclude the discussion with the overall comparison of all methods and potential directions for future work. 

% \subsubsection{Analytical Optimization-based Methods}

% As illustrated in the Table~\ref{optimization_table_results} and the Figure~\ref{fig:plot_losses_optmimization}, there is no silver bullet consistently outperforming others in the context of analytical optimization-based approaches. The SHGO-SDF and BH-SDF methods show a solid performance for problems with a small number of variables. However, as the complexity increases with more optimization variables, the methods struggle, failing to produce good enough results, as seen in the Gyroid~[5D] case, or even SHGO-SDF not yielding any results for the Porous~[28D]. A significant limitation is their sensitivity to hyperparameters. To get the results of the SHGO-SDF and BH-SDF, we had to rerun the optimization multiple times for each case, using different
% hyperparameters and random seeds, making the optimization quite tedious and expensive. Additionally, their need for differentiability of the fitting function $f$ makes it unusable for certain problems, such as the Spheres~[2D]. Another drawback of SHGO-SDF is its unstable convergence behavior, as seen in the Figure~\ref{fig:plot_losses_optmimization}, which leaves the user uncertain about whether the optimizer is approaching a solution, complicating the interpretation of its progress. Likewise, BH-SDF exhibits the same flaw, however BH-SDF shows a slightly more stable convergence behavior, though this depends on the problem, as demonstrated by two different convergence plots for BH-SDF in the Figure~\ref{fig:plot_losses_optmimization}. BH-SDF might also be, to some degree, more suitable for multi-variable problems compared to SHGO-SDF. This is demonstrated on the Porous~[28D], where SHGO-SDF completely fails, while the BH-SDF at least returns some result. Finally, the CMA-ES-SDF method performs reasonably well even for higher-dimensional as well as for smaller-scale problems. The hyperparameters, i.e. the population size and $\sigma_0$ are intuitive to tune. For more complex problems, simply increasing $\sigma_0$ and the population size often yields better results, making the method user-friendly in terms of parameter selection.
% The nature of the evolutionary algorithm of not requiring a differentiability of the fitting function $f$ are important advantages. Additionally, it exhibits a steady convergence rate making it more informative for the user during the training.  However, it also fails even in certain smaller-scale scenarios, such as the Fibers~[2D] and the Gyroid~[3D]. This is due to a higher proneness to local minima, which can be seen, for example, in the Fibers~[2D] example in Figure~\ref{fig:plot_losses_optmimization}. Overall, we suggest working with SHGO-SDF and BH-SDF for small-dimensional problems (when applicable) and using CMA-ES-SDF for non-differentiable or higher-dimensional problems.

% \subsubsection{Analysis-by-Synthesis Methods}

% In the analysis-by-synthesis methods, as seen in the Table~\ref{optimization_table_results} and in the Figure~\ref{fig:plot_losses_optmimization}, there is a little difference between the Powell-S and CMA-ES-S methods. Both are very slow, and are only able to solve the gyroid family problems. Although, the Gyroid~[5D] problem can be solved only with CMA-ES-S and CMA-ES-SDF methods, making the analysis-by-synthesis useful in certain scenarios. Furhermore, they do have the advantage of being applicable to non-differentiable cases, such as the Spheres [2D]. If any preference is to be given, Powell-S has a small advantage over CMA-ES-S. While it is more sensitive to the initial value than the CMA-ES-S method, it requires no hyperparameter tuning beyond the initial value $\boldsymbol{\phi}_0$, and also requires fewer evaluations. It is also important to note that analysis-by-synthesis is a more challenging problem to solve compared to the other two signed distance value fitting approaches, as its only input is the RGB image. Despite this limitation, we think it can achieve good results in certain cases, as the image loss may provide more information for parameter tuning. For this reason, we think the approach has yet unexplored potential.

% \subsubsection{Approaches Comparison}

% The Figure~\ref{fig:plot_losses_optmimization} clearly shows that the number of iterations required for analytical optimization-based methods is significantly higher compared to analysis-by-synthesis approaches. However, as seen in Table~\ref{optimization_table_results}, the analytical methods are considerably faster. Furthermore, the render comparisons demonstrate that the analytical optimization-based methods produce better results than the analysis-by-synthesis methods. Although, it is important to note that we are not able to solve the high-dimensional Porous~[28D] with any of the current artillery. In conclusion, the analytical optimization-based methods achieve the best overall performance, outperforming the analysis-by-synthesis methods. 


% \subsection{Future Work}

% As previously discussed, no analytical optimization-based method serves as a one-size-fits-all solution. Ideally, future work could treat the choice of optimizer itself as a hyperparameter within a multi-threaded system, where different methods are applied simultaneously. This could be further extended by incorporating analysis-by-synthesis methods as an additional stage in the optimization pipeline, particularly for handling non-differentiable problems. 

% Another major limitation, however, is the sensitivity of the \ac{BH} and \ac{SHGO} optimizers to hyperparameters. A potential solution to address this would be adding another hypothetical stage to the system. This process would involve rerunning the optimization multiple times with a set of empirically determined, high-quality hyperparameters of the optimizers. Each stage would progressively analyse the quality of hyperparameters based on previous results, eventually returning only the solution with the smallest loss. 

% Finally, our inability to solve high-dimensional problems, highlights the need for more research into better global optimizers and improved loss function formulations. Potentially, next step could be to reformulate the problem as a simpler linear system of equations $\mathbf{Ax = b}$ and solve it using the recently developed learned preconditioning of the conjugate gradient~\cite{li2023learning}. Another promising direction could involve an iterative two-phase optimization approach: first, a 1D optimization of the noise-scale parameter, followed by optimizing the remaining parameters. This idea comes from the fact that the noise-scale influences every microstructure \ac{SDF} and has a significant impact on the visuals, often more so than the other parameters. 

% What's more, we find a big potential in the analysis-by-synthesis methods. However, the results show that the gradient-free optimization is not sufficient. Moving forward, we could either transform our pipeline to a differentiable one using for instance\cite{vicini2022differentiable, liu2020dist, jiang2020sdfdiff}, or potentially apply the surrogate loss using the ZeroGrads~\cite{fischer2024zerograds} on our analysis-by-synthesis loss.

% Furthermore, it would be worth exploring some \acp{INR}, such as the network with Gabor wavelet activation function~\cite{saragadam2023wire} or the \ac{MLP} with a trainable multiresolution hash encoding~\cite{muller2022instant}. A novel perspective on \acp{MLP} is offered by the \acp{KAN}~\cite{liu2024kan} which, according to the authors, should be superior to the tradional \ac{MLP} architecture. Another advantage of \acp{KAN} is their explainability, which allows the network to be reduced to an analytical formula. This could be a tool to discovering new \ac{SDF} representations of microstructures. An interesting direction of future research could also be to compare our \acp{INR} with the 1-Lipschitz Neural Distance Fields~\cite{coiffier20241}. 

% In addition, we believe that additional comparison metrics for microstructures could be introduced. The metrics we used tend to penalize small changes in linear transformations, which are unimportant in microstructure reconstruction. This is evident in the Figure~\ref{tab:comparison_contd}, in the example of the Gyroid[5D] when comparing CMA-ES-SDF and BH-SDF. One option is to fine-tune the \ac{LPIPS} network on the microstructure exemplars. 

% Finally, we would like to extend our microstructure dataset with real microstructures extracted from the \ac{microCT}. To obtain the signed distance fields from a real world CT scan, we could for instance adapt the technique introduced in \cite{park2019deepsdf}. To get the ground truth exemplar for the analysis-by-synthesis methods, any suitable render of the microstructure's \ac{microCT} scan image, where the patterns are clearly visible, can be used as the target, as long as the parameters $\mathbf{K}$ and $\mathbf{E}$ stay fixed and the shading somewhat corresponds to the \ac{BRDF} in the pipeline $\mathcal{R}$.

\subsection{Synthetic Dataset}
\label{synthetic_dataset}

\begin{figure}[ht]
    \centering
    \begin{adjustbox}{max width=\textwidth, max height=0.17\textheight}
    \setlength{\tabcolsep}{1.5pt} % Adjust column separation
    \renewcommand{\arraystretch}{0.3} % Adjust row separation
    \begin{tabular}{c c c}
        \includegraphics[width=0.15\textwidth]{figures/optimization_results/fitting_render-0_resized.png} &
        \includegraphics[width=0.15\textwidth]{figures/optimization_results/fitting_render-1.png} &
        \includegraphics[width=0.15\textwidth]{figures/optimization_results/fitting_render-2.png}\\
        \includegraphics[width=0.15\textwidth]{figures/optimization_results/fitting_render-3.png} &
        \includegraphics[width=0.15\textwidth]{figures/optimization_results/fitting_render-4.png} &
        \includegraphics[width=0.15\textwidth]{figures/optimization_results/fitting_render-5.png} 
    \end{tabular}
    \end{adjustbox}
    \caption{Instances of exemplar renders (\textit{top row}) Gyroid~[1D] \ref{gyroid1d}, Fibers~[2D] \ref{fibers_sdf}, Gyroid~[3D] \ref{gyroid3d} respectively. Rest of the renders (\textit{bottom row}) are Spheres~[2D]~\ref{sphere_microstructure}, Gyroid~[5D] \ref{gyroid5d}, Porous~[28D]~\ref{porous_material_sdf} respectively.}
    \label{tab:renders_exemplars}
\end{figure}

For the proof of concept and more control over the experiments, we test our algorithms on representative synthetic examples that closely resemble SEM/TEM images. Let us now describe our synthetic dataset of microstructures. The dataset consists of six microstructures. Each microstructure is defined by a SDF $\hat{f}$ with $n$ parameters, denoted as $\boldsymbol{\phi}$ in Approaches~\ref{parameter_fitting_approach} and~\ref{analysis_by_synthesis_approach}. We include the number of parameters inside square brackets in the naming conventions to reflect both the degrees of freedom and to provide an indication of the optimization complexity. All ground-truth parameter values presented in the dataset were selected for their convenience and to ensure they fit in the defined domain range.

\subsubsection{Gyroid Family}  

The first family of microstructures are the gyroid microstructures. These consist of periodic fully deterministic patterns created using trigonometric functions. Our dataset includes three such microstructures with 1, 3, 5 degrees of freedom respectively. 

The simplest example is the Gyroid [1D]. The only parameter is a scalar variable $\eta \in \mathbb{R}$. We call $\eta$ the noise scale. The $\eta$ variable controls the density of the microgeometry. We create the ground-truth using $\eta = 100$:

\begin{equation}
\hat{f}(\mathbf{x} \mid \eta) = \sum_i^3{\sin(x_i \cdot \eta )} / \eta.
\label{gyroid1d}
\end{equation}

The second element from the set of gyroid functions, Gyroid [3D], is guided by $\eta \in \mathbb{R}$, and $k = 2 \cdot \pi / a \in \mathbb{R}, t \in \mathbb{R}$. The $a$ represents the cell size of the gyroid structure, $t$ represents the wall thickness. 
We create the ground-truth using the setting of $\eta = 100.0$, $a = 7.0$, $t = 1.2$ as follows
\begin{gather}
 \label{gyroid3d}
 \hat{f}(\mathbf{x} \mid \eta, k, t  ) = g(\mathbf{x} \cdot \eta \mid k, t  ) / \eta ,\\
 \notag\\
g(\mathbf{x} \mid k, t ) = \sin(k x_0)\cos(k x_1)+ \\ \sin(k x_1)\cos(kx_2)+\sin(kx_2)\cos(kx_0)+t.
\end{gather}
Finally, the last exemplar, the Gyroid [5D], closely resembles the Gyroid [3D] problem. The only difference is the division of the $\mathbf{a} \in \mathbb{R}^3$ parameter into three variables $k_i = 2 \cdot \pi / a_i$, each controlling the cell size of the gyroid in the $x$, $y$, and $z$ directions. We create the ground-truth using the setting $\eta = 100.0$, $\mathbf{a} = (7.0, 10.0, 15.0)$, $t = 1.2$. The fitting is again thus: 
\begin{gather}
\label{gyroid5d}
\hat{f}(\mathbf{x} \mid \eta, \mathbf{k}, t ) = r(\mathbf{x} \cdot \eta \mid \mathbf{k}, t  ) / \eta, \\
\notag\\
r(\mathbf{x} \mid \mathbf{k}, t ) = \sin(k_1 x_0)\cos(k_2 x_1)+ \\ \sin(k_2 x_1)\cos(k_3 x_2)+\sin(k_3 x_2)\cos(k_1 x_0)+t,
\end{gather}
Note that the $\hat{f}$ is, in all cases, differentiable, thus enabling the use of first-order optimization. 

\subsubsection{Spherical Microstructure}

Our next microstructure consists of a signed distance function for randomly placed spheres. We generate a granular material microgeometry; to achieve this, we use a space-filling grid-based random variable of points. A grid cell index, which is computed from its floored location, is used to generate a seed $t$ for PRNG. A multilinear hash function defining the seed looks as follows:

\begin{equation}
t_l(\mathbf{x}) = M \sum_{i=0}^1 \sum_{j=0}^1 \sum_{k=0}^1 a_{ijk} q_l(x_0)^i q_l(x_1)^j q_l(x_2)^k,    
\end{equation}

where $(q_l(x_0), q_l(x_1), q_l(x_2))$ are grid indices generated in eight possible directions by adding binary-encoded offsets, dependent on $l$, to the base grid coordinates computed from the floored location $\eta \cdot \mathbf{x}$ which is noise-scale $\eta$ dependent. $M$ and all $a_{ijk}$ were selected such that regularity artifacts are avoided.  
Seed $t_l$ is later used as an input to PRNG, generating a pseudo-random number in the interval~$[0, 1)$. We then add the randomly generated number to the grid position to obtain the center of a random sphere in the current grid. We repeat the described procedure in total 8 times (once for each potential overlapping grid cell). Finally, the signed distance is calculated by finding a minimum distance to all spheres taking into account their radius. The variables are the density-controlling $\eta \in \mathbb{R}$ and the radius of the spheres $r \in \mathbb{R}$. Mathematically, the procedure looks as follows
\begin{gather}   
\label{sphere_microstructure}
\hat{f}(\boldsymbol{x} \mid \eta, r ) = \Bigl( \min_{l=1}^8 || c_l(\eta \cdot\mathbf{x}, t_l(\eta \cdot\mathbf{x})) - \mathbf{x} ||_2  - r \Bigr) / \eta,    \\
c_l(\eta \cdot\mathbf{x}, t_l(\eta \cdot\mathbf{x})) = \mathbf{q}_l(\eta \cdot\mathbf{x}) + \text{PRNG}(t_l(\eta \cdot\mathbf{x})), \\
\mathbf{q}_l(\eta \cdot \mathbf{x}) = \lfloor \eta \cdot \mathbf{x} \rfloor + \mathcal{U}_l, 
\end{gather}

where $\mathbf{x}, t_i(\mathbf{x}), c(\mathbf{x}, t_i(\mathbf{x}))$, $\mathcal{U}_l$ are a point of evaluation, generated random seed, generated center of a random sphere, and $l$-th element of the unit cube vertices $\mathcal{U} = \{ (v_1, v_2, v_3)  \mid v_i \in \{0, 1\}\}$, respectively. We use the following setting to create the ground-truth $\eta = 30.0$, $r = 0.08$.

The $\mathbf{q}_l(\eta \cdot \mathbf{x})$ is computed by flooring the point coordinates, which eliminates the gradient with respect to $\eta$ entirely. Additionally, the center is calculated by adding a random value $\text{PRNG}(t_l(\eta \cdot\mathbf{x}))$ to the grid. However, the PRNG is not differentiable, making $\hat{f}$ a non-differentiable function.

To maintain consistency between the Python implementation of the signed distance field generation, defined by the Equation~\ref{sphere_microstructure},  and the rendering of the microstructure, given by the same equation and processed within a CUDA shader, the CUDA PRNG is called directly from Python. This ensures both environments use the same random number generation process, avoiding potential differences in results.
 
\subsubsection{Fibers Microstructure}

Next, we describe a procedure to obtain a union of two rotated sets of fibers parallel to the y-axis arranged in layers. To achieve this, we need a rotation transformation matrix $T_\varphi$ along the axis y by an angle $\varphi \in [0, 2\pi]$, which is a parameter. Thanks to the symmetry of the problem, we can constrain the $\varphi \in [0, \pi]$.  We also need a function $u : \mathbb{R}^3 \rightarrow \mathbb{R}$ defining the fibers. The last parameter is the $\eta \in \mathbb{R}$ controlling the density of the fibers. The microstructure Fibers [2D] is defined by
\begin{gather}
\label{fibers_sdf}
 \hat{f}(\mathbf{x} | \eta, \phi ) =  h(\mathbf{x} \cdot \eta | \phi) / \eta, \\
 \notag\\
 h(\mathbf{x} | \phi ) = \min \Bigl( u(\mathbf{x}) + u((x_1, x_1, x_1)) , u(T_\phi(\mathbf{x})) + u(T_\phi(x_1, x_1, x_1)) \Bigr), \\
  \notag\\
u(x) = (\sin(x_0)\cos(x_1)+\sin(x_1)\cos(x_2)+\sin(x_2)\cos(x_0))^2 .   
\end{gather}

Note that all functions used are periodic functions and linear transformations, all of which are differentiable, making the $\hat{f}$ also differentiable. To create the ground truth, we set $\eta = 100, \varphi = \pi / 4$.


\subsubsection{Porous Microstructure}
\label{porous_material}

Lastly, we present the function defining a porous microstructure named Porous [28D]. The first parameter, $\eta \in \mathbb{R}$, controls the density of the material. The SDF is composed of a summation of various sine and cosine waves with different amplitudes and frequencies, resulting in a complex material structure. The frequencies are determined by three $3\times3$ parameter transformation matrices, simplified as $\mathbf{T} \in \mathbb{R}^{3\times 3 \times 3}$. The final distance is then given by
\begin{gather}
\label{porous_material_sdf}
\hat{f}(\mathbf{x} | \eta, \mathbf{T}) = \min \Bigl(\epsilon, v(\eta\mathbf{T}_1 \mathbf{x}) + w(\eta\mathbf{T}_2 \mathbf{x}) \cdot v(\eta\mathbf{T}_3 \mathbf{x}) \Bigr) / \eta, \\
v(\mathbf{x}) = \Bigl( \sin(x_0) \cos(x_1) + \sin(x_1) \cos(x_2) + \sin(x_2) \cos(x_0) \Bigr)^2, \\
w(\mathbf{x}) = \Bigl( \sin(x_0) \sin(x_1) + \sin(x_1) \sin(x_2) + \sin(x_2) \sin(x_0) \Big)^2,
\end{gather}

where $\epsilon$ is a small positive number. The $\hat{f}$ is again differentiable thanks to a differentiability of composition of linear transformations and periodic functions. The ground truth is created with a fixed $\eta = 30$ and the $\mathbf{T} \in [-4, 7]^{3\times 3 \times 3}$.

\subsection{Results}

\definecolor{darkorange}{RGB}{255,140,0}  % RGB values for dark orange


\begin{table*}[ht]
\begin{adjustbox}{max width=\textwidth, max height=0.2\textheight, center}
\begin{tabular}{l r | >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm}} 
Microstructure & & SHGO-SDF & BH-SDF & CMA-ES-SDF & CMA-ES-S & Powell-S\\
\toprule
    % \multirow{5}{*}{Gyroid [1D]} & MAPE$\downarrow$ & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$\% & \cellcolor{orange!25}$\mathbf{1\times10^{-3}\%}$ & \cellcolor{orange!25}$\mathbf{4\times10^{-2}}\%$ & 14.6\% & 0.53\%\\ 
    \multirow{5}{*}{Gyroid [1D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & $10^{-4}$ & \cellcolor{yellow!25}$10^{-6}$\\ 
& LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{orange!25}\textbf{0.00}& \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.02 & \cellcolor{orange!25}\textbf{0.00}\\ 
& \FLIP$\downarrow$ &  \cellcolor{yellow!25}$3\times10^{-7}$  & \cellcolor{orange!25}$\mathbf{1\times10^{-7}}$ &  $1\times10^{-3}$  &  $2\times10^{-3}$ &  $2\times10^{-3}$\\ 
& Time$\downarrow$ & \cellcolor{orange!25}\textbf{2.85s}  & \cellcolor{yellow!25}16.67s & \cellcolor{orange!25}\textbf{2.23s}  & 20m & 7m\\ 
& $\Delta$-loss$\uparrow$ & 23.67 & 23.87 & 19.25  & 4.55 & 8.12 \\
\\
% \multirow{5}{*}{Fibers [2D]} & MAPE$\downarrow$ & 106.03\% & \cellcolor{orange!25}\textbf{2.55}\% & 487.82\% & 693.64\% & 806.59 \%\\ 
\multirow{5}{*}{Fibers [2D]} & Val. Error$\downarrow$ & \cellcolor{yellow!25}0.34 & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & 0.65 & 1.00 & 1.00\\ 
& LPIPS$\downarrow$ & \cellcolor{yellow!25}0.41 & \cellcolor{orange!25}\textbf{0.13} & 0.54 & 0.56 & 0.56   \\ 
& \FLIP$\downarrow$ &  \cellcolor{yellow!25}0.3  & \cellcolor{orange!25}\textbf{0.14} & 0.42  &  0.40 &  0.43 \\ 
& Time$\downarrow$ & 13m  & 20m & \cellcolor{yellow!25}6m  & 20m & \cellcolor{orange!25}\textbf{5m}\\ 
& $\Delta$-loss$\uparrow$   & 2.17 & 7.58 & 1.46  & 0.08 & 0.05 \\ 
\\
% \multirow{5}{*}{Gyroid [3D]} & MAPE$\downarrow$ & 0.07\% & \cellcolor{orange!25}\textbf{0.01\%} & 1893.16\%& 346.27\% & 7.46\%\\ 
\multirow{5}{*}{Gyroid [3D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & $6\times10^{-3}$ & 1.02& 0.15 & \cellcolor{yellow!25}$2\times10^{-3}$\\ 
& LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.01} & 0.04 & 0.65 & 0.35 & \cellcolor{yellow!25}0.02\\ 
& \FLIP$\downarrow$ &  \cellcolor{orange!25}\textbf{0.01}  & 0.05 &  0.61 &  0.42 &  \cellcolor{yellow!25}0.03 \\ 
& Time$\downarrow$ & \cellcolor{orange!25}\textbf{22.7s} & 20m & \cellcolor{yellow!25}7m & 14m & 20m\\ 
& $\Delta$-loss$\uparrow$   & 18.2 & 18.88 & 0.72& 1.64 & 4.66 \\ 
\\
\multirow{5}{*}{Spheres [2D]} & Val. Error$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}$\mathbf{1\times10^{-5}}$ & 1.01 & 1.01\\ 
& LPIPS$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{0.00} & 0.53 & 0.53\\ 
& \FLIP$\downarrow$ &  \sout{N/A}& \sout{N/A} & \cellcolor{orange!25}$\mathbf{3\times10^{-7}}$  &  0.55 & 0.55 \\ 
& time$\downarrow$ &\sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{4m}  & 20m & 5m\\ 
& $\epsilon$-loss$\uparrow$  & \sout{N/A} &\sout{N/A} & 11.34  & 0.63 & 0.61 \\ 
\\
\multirow{5}{*}{Gyroid [5D]} & Val. Error$\downarrow$ & 0.66 & 0.65 & \cellcolor{orange!25}\textbf{$\mathbf{3\times10^{-4}}$} & \cellcolor{yellow!25}0.03 & 0.44 \\ 
& LPIPS$\downarrow$ & 0.42 & 0.57 & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.21 & 0.54 \\ 
& \FLIP$\downarrow$ &  0.42  & 0.62 &  \cellcolor{orange!25}\textbf{$\mathbf{6\times10^{-3}}$}  &  \cellcolor{yellow!25}0.28 &  0.60\\ 
& Time$\downarrow$ & \cellcolor{orange!25}\textbf{2m} & 15m & \cellcolor{yellow!25}11m  & 20m & 15m \\ 
& $\Delta$-loss$\uparrow$  & 1.92 & 1.75 & 20.34  & 2.14 & 1.60\\ 
\\
\multirow{5}{*}{Porous [28D]} & Val. Error$\downarrow$ & \sout{N/A} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00}\\ 
& LPIPS$\downarrow$ & \sout{N/A} & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{orange!25}\textbf{0.61}\\ 
& \FLIP$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{0.51} & \cellcolor{yellow!25}0.52 & \cellcolor{yellow!25}0.52 & 0.59\\ 
& Time$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{4m} & \cellcolor{yellow!25}8m & 20m & 20m\\ 
& $\Delta$-loss$\uparrow$  & \sout{N/A} & 0.88 & 0.01 & 1.6 & 0.23\\ 
\end{tabular}
\end{adjustbox}
\caption{Fitted Functions. Table of comparison of the global optimization algorithms used on our synthetic dataset~\ref{synthetic_dataset}. We show for each problem the following: \textbf{a)} Validation Error, \textbf{b)} LPIPS Perceptual loss, \textbf{c)} \FLIP error, \textbf{d)} Time of the optimization, \textbf{e)} The difference between the loss at the beginning and at the end of the optimization process is denoted as $\Delta$-loss. The time limit for all examples was set to 20 minutes. We consider a numerical~0 to be a number below $1\times10^{-7}$. The \sout{N/A} implies that the method could not be used for the problem. }
\label{optimization_table_results}
\end{table*}



\definecolor{darkorange}{RGB}{0,0,0}  % RGB values for dark orange
\begin{table*}[ht]
\begin{adjustbox}{max width=\textwidth, max height=0.4\textheight}
\begin{tabular}{ |c c c||c|c|c|c|c| } 
\hline
Problem & Ground Truth & Init. & SHGO-A  & BH-A & CMA-ES-A & CMA-ES-S & Powell-S\\
\hline
\hline
\multirow{1}{*}{Gyroid [1D]} & $\eta$: 100.0 & 300.0 & \cellcolor{orange!25}\textbf{100.000} & \cellcolor{orange!25}\textbf{100.000} & \cellcolor{orange!25}\textbf{100.000} & 100.001 & \cellcolor{orange!25}\textbf{100.000}\\ 
\hline
\multirow{2}{*}{Fibers [2D]} & $\eta$: 100.0 & 200.0 & \cellcolor{orange!25}\textbf{100.000} & \cellcolor{orange!25}\textbf{100.000} & 100.100 & 175.159 &  133.202\\ 
& $\theta: \pi / 4$  &  $\pi$ & 0.142 &  \cellcolor{orange!25}\textbf{0.785} &  2.825 &  3.126 &  0.831\\
\hline
\multirow{3}{*}{Gyroid [3D]} & 
$\eta$: 100.0 & 300.0 &  \cellcolor{orange!25}\textbf{116.633} &  213.469 & 32.000 & 186.593 & 86.780 \\ 
& $a: 7.0$  & 6.0 &  8.164 &  14.942 &  11.010 &  12.958 &  \cellcolor{orange!25}\textbf{6.075}\\
& $t: 1.2$  & 0.0 &  \cellcolor{orange!25}\textbf{1.200} &  \cellcolor{orange!25}\textbf{1.200}  &  1.196 &  1.173 & 1.198 \\
\hline
\multirow{2}{*}{Spheres [2D]} & 
$\eta$: 30.0 & 150.0 & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{29.999} & 291.739 & 300.964  \\ 
& $r: 0.08$  & 0.2 &  \sout{N/A} &  \sout{N/A} &  \cellcolor{orange!25}\textbf{0.079} &  0.093 &  0.086\\
\hline
\multirow{5}{*}{Gyroid [5D]} & 
$\eta$: 100.0 & 200.0 &  114.983 & 142.570 & \cellcolor{orange!25}\textbf{97.668} & 74.162 & 89.104 \\ 
& $a: 7.0$  & 6.0 &  8.051 &  9.979 &  \cellcolor{orange!25}\textbf{6.836} &  5.180 &  6.319\\
& $t: 10.0$  & 6.0 &  11.534 &  14.162  &  \cellcolor{orange!25}\textbf{9.766} &  7.376 & 9.228 \\
& $t: 15.0$  & 6.0 &  \cellcolor{orange!25}\textbf{14.961} &  14.778  &  14.650 &  11.062 & 13.125 \\
& $t: 1.2$  & 6.0 &  1.180 &  1.199  &  \cellcolor{orange!25}\textbf{1.200} &  1.165 & 1.151 \\
\hline
\multirow{1}{*}{Porous [28D]} & 
$\eta$: 30.0 & 50.0 &  \sout{N/A} & 38.586 & 42.796 & \cellcolor{orange!25}\textbf{28.268}  & 43.272 \\ 
\hline
\end{tabular}
\end{adjustbox}
    \caption{Optimal function parameters $\boldsymbol{\phi}$ Table. Optimal parameters found by the specified global optimizers. These results refer to the Table~\ref{optimization_table_results}. The parameters were rounded to 3 decimal points. We also specify the ground truth and the initialization of the variables.}
\label{optimization_table_parameters}
\end{table*}

%{l r | >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm}} 
% \begin{table}[ht]
% \begin{adjustbox}{max width=\textwidth, max height=0.2\textheight, center}
% \begin{tabular}{l r | c c c c} 
% Microstructure & Metrics & SHGO-SDF & BH-SDF & CMA-ES-SDF \\
% \toprule
% \multirow{5}{*}{Gyroid [1D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ \\ 
% & LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{orange!25}\textbf{0.00}& \cellcolor{orange!25}\textbf{0.00} \\ 
% & \FLIP$\downarrow$ &  \cellcolor{yellow!25}$3\times10^{-7}$  & \cellcolor{orange!25}$\mathbf{1\times10^{-7}}$ &  $1\times10^{-3}$  \\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{2.85s}  & \cellcolor{yellow!25}16.67s & \cellcolor{orange!25}\textbf{2.23s} \\ 
% & $\Delta$-loss$\uparrow$ & 23.67 & 23.87 & 19.25  \\
% \\
% \multirow{5}{*}{Fibers [2D]} & Val. Error$\downarrow$ & \cellcolor{yellow!25}0.34 & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & 0.65 \\ 
% & LPIPS$\downarrow$ & \cellcolor{yellow!25}0.41 & \cellcolor{orange!25}\textbf{0.13} & 0.54  \\ 
% & \FLIP$\downarrow$ &  \cellcolor{yellow!25}0.3  & \cellcolor{orange!25}\textbf{0.14} & 0.42  \\ 
% & Time$\downarrow$ & 13m  & 20m & \cellcolor{yellow!25}6m  \\ 
% & $\Delta$-loss$\uparrow$   & 2.17 & 7.58 & 1.46  \\
% \\
% \multirow{5}{*}{Gyroid [3D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & $6\times10^{-3}$ & 1.02 \\ 
% & LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.01} & 0.04 & 0.65 \\ 
% & \FLIP$\downarrow$ &  \cellcolor{orange!25}\textbf{0.01}  & 0.05 &  0.61  \\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{22.7s} & 20m & \cellcolor{yellow!25}7m \\ 
% & $\Delta$-loss$\uparrow$   & 18.2 & 18.88 & 0.72\\ 
% \\
% \multirow{5}{*}{Gyroid [5D]} & Val. Error$\downarrow$ & 0.66 & 0.65 & \cellcolor{orange!25}\textbf{$\mathbf{3\times10^{-4}}$} \\ 
% & LPIPS$\downarrow$ & 0.42 & 0.57 & \cellcolor{orange!25}\textbf{0.00} \\ 
% & \FLIP$\downarrow$ &  0.42  & 0.62 &  \cellcolor{orange!25}\textbf{$\mathbf{6\times10^{-3}}$}  \\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{2m} & 15m & \cellcolor{yellow!25}11m  \\ 
% & $\Delta$-loss$\uparrow$  & 1.92 & 1.75 & 20.34  \\
% \\
% \multirow{5}{*}{Porous [28D]} & Val. Error$\downarrow$ & \sout{N/A} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} \\ 
% & LPIPS$\downarrow$ & \sout{N/A} & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 \\ 
% & \FLIP$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{0.51} & \cellcolor{yellow!25}0.52 \\ 
% & Time$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{4m} & \cellcolor{yellow!25}8m \\ 
% & $\Delta$-loss$\uparrow$  & \sout{N/A} & 0.88 & 0.01 \\ 
% \end{tabular}
% \end{adjustbox}
% \caption{Fitted Functions. Table of comparison of the global optimization algorithms used on our synthetic dataset.}
% \label{optimization_table_results1}
% \end{table}

% \definecolor{darkorange}{RGB}{255,140,0}  % RGB values for dark orange
% \begin{table}[ht]
% \begin{adjustbox}{max width=\textwidth, max height=0.2\textheight, center}
% \begin{tabular}{l r | >{\centering\arraybackslash}m{2.5cm} >{\centering\arraybackslash}m{2.5cm}} 
% Microstructure & Metrics & CMA-ES-S & Powell-S\\
% \toprule
%     \multirow{5}{*}{Gyroid [1D]} & Val. Error$\downarrow$ & $10^{-4}$ & \cellcolor{yellow!25}$10^{-6}$\\ 
% & LPIPS$\downarrow$ & \cellcolor{yellow!25}0.02 & \cellcolor{orange!25}\textbf{0.00}\\ 
% & \FLIP$\downarrow$ &  $2\times10^{-3}$ &  $2\times10^{-3}$\\ 
% & Time$\downarrow$ & 20m & 7m\\ 
% & $\Delta$-loss$\uparrow$ & 4.55 & 8.12 \\
% \\
% \multirow{5}{*}{Fibers [2D]} & Val. Error$\downarrow$ & 1.00 & 1.00\\ 
% & LPIPS$\downarrow$ & 0.56 & 0.56   \\ 
% & \FLIP$\downarrow$ &  0.40 &  0.43 \\ 
% & Time$\downarrow$ & 20m & \cellcolor{orange!25}\textbf{5m}\\ 
% & $\Delta$-loss$\uparrow$   & 0.08 & 0.05 \\
% \\
% \multirow{5}{*}{Gyroid [3D]} & Val. Error$\downarrow$ & 0.15 & \cellcolor{yellow!25}$2\times10^{-3}$\\ 
% & LPIPS$\downarrow$ & 0.35 & \cellcolor{yellow!25}0.02\\ 
% & \FLIP$\downarrow$ &  0.42 &  \cellcolor{yellow!25}0.03 \\ 
% & Time$\downarrow$ & 14m & 20m\\ 
% & $\Delta$-loss$\uparrow$   & 1.64 & 4.66 \\
% \\
% \multirow{5}{*}{Spheres [2D]} & Val. Error$\downarrow$ & 1.01 & 1.01\\ 
% & LPIPS$\downarrow$ & 0.53 & 0.53\\ 
% & \FLIP$\downarrow$ &  0.55 & 0.55 \\ 
% & time$\downarrow$ & 20m & 5m\\ 
% & $\epsilon$-loss$\uparrow$  & 0.63 & 0.61 \\
% \\
% \multirow{5}{*}{Gyroid [5D]} & Val. Error$\downarrow$ & \cellcolor{yellow!25}0.03 & 0.44 \\ 
% & LPIPS$\downarrow$ & \cellcolor{yellow!25}0.21 & 0.54 \\ 
% & \FLIP$\downarrow$ &  \cellcolor{yellow!25}0.28 &  0.60\\ 
% & Time$\downarrow$ & 20m & 15m \\ 
% & $\Delta$-loss$\uparrow$  & 2.14 & 1.60\\
% \\
% \multirow{5}{*}{Porous [28D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00}\\ 
% & LPIPS$\downarrow$ & \cellcolor{yellow!25}0.64 & \cellcolor{orange!25}\textbf{0.61}\\ 
% & \FLIP$\downarrow$ & \cellcolor{yellow!25}0.52 & 0.59\\ 
% & Time$\downarrow$ &  20m & 20m\\ 
% & $\Delta$-loss$\uparrow$  & 1.6 & 0.23\\ 
% \end{tabular}
% \end{adjustbox}
% \caption{Fitted Functions. Table of comparison of the global optimization algorithms used on our synthetic dataset~\ref{synthetic_dataset}. We show for each problem the following: \textbf{a)} Validation Error~\ref{validation_error}, \textbf{b)} LPIPS Perceptual loss, \textbf{c)} \FLIP error, \textbf{d)} Time of the optimization, \textbf{e)} The difference between the loss at the beginning and at the end of the optimization process denoted as $\Delta$-loss. The time limit for all examples was set to 20~minutes. We consider a numerical~0 to be a number below $1\times10^{-7}$. }
% \label{optimization_table_results2}
% \end{table}

In Table \ref{optimization_table_results}, we report the performance of different algorithms for different microstructures. In Fig. \ref{fig:reconstruction_renders}, we show the corresponding renders. We set a maximum time limit for the optimization of approximately 20 minutes, as results typically do not improve significantly beyond this point. The results show that no single optimization algorithm consistently outperforms the others across all microstructures. SHGO-SDF and BH-SDF perform well for small-variable problems but struggle with higher-dimensional cases (e.g., Gyroid [5D], Porous [28D]) and cannot be applied to certain discrete problems (e.g., Spheres [2D]). CMA-ES-SDF demonstrates solid performance across different microstructures, including discrete ones like Spheres [2D]. As expected, parameter fitting methods outperform analysis-by-synthesis in both accuracy and efficiency, given the larger complexity of the latter. Interestingly, CMA-ES-S resemble more Porous [28D] more than the other methods, highlighting its potential for high-dimensional reconstructions.\\

In Table \ref{optimization_table_results}, we report the performance of different algorithms for different microstructures. In Fig. \ref{fig:reconstruction_renders}, we show the corresponding renders. We set a maximum time limit for the optimization of approximately 20 minutes, as results typically do not improve significantly beyond this point. The results show that no single optimization algorithm consistently outperforms the others across all microstructures. SHGO-SDF and BH-SDF perform well for small-variable problems but struggle with higher-dimensional cases (e.g., Gyroid [5D], Porous [28D]) and cannot be applied to certain discrete problems (e.g., Spheres [2D]). CMA-ES-SDF demonstrates solid performance across different microstructures, including discrete ones like Spheres [2D]. As expected, parameter fitting methods outperform analysis-by-synthesis in both accuracy and efficiency, given the larger complexity of the latter. Interestingly, CMA-ES-S resamble more Porous [28D] more than the other methods, highlighting its potential for high-dimensional reconstructions.\\

%\definecolor{darkorange}{RGB}{255,140,0}  % RGB values for dark orange
% \begin{table}[ht]
% \begin{adjustbox}{max width=\textwidth, max height=0.2\textheight, center}
% \begin{tabular}{l r | c c c c c} 
% Microstructure & Metrics & SHGO-SDF & BH-SDF & CMA-ES-SDF & CMA-ES-S & Powell-S\\
% \toprule
%     \multirow{5}{*}{Gyroid [1D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & $10^{-4}$ & \cellcolor{yellow!25}$10^{-6}$\\ 
% & LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{orange!25}\textbf{0.00}& \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.02 & \cellcolor{orange!25}\textbf{0.00}\\ 
% & \FLIP$\downarrow$ &  \cellcolor{yellow!25}$3\times10^{-7}$  & \cellcolor{orange!25}$\mathbf{1\times10^{-7}}$ &  $1\times10^{-3}$  &  $2\times10^{-3}$ &  $2\times10^{-3}$\\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{2.85s}  & \cellcolor{yellow!25}16.67s & \cellcolor{orange!25}\textbf{2.23s}  & 20m & 7m\\ 
% & $\Delta$-loss$\uparrow$ & 23.67 & 23.87 & 19.25  & 4.55 & 8.12 \\
% \\
% \multirow{5}{*}{Fibers [2D]} & Val. Error$\downarrow$ & \cellcolor{yellow!25}0.34 & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & 0.65 & 1.00 & 1.00\\ 
% & LPIPS$\downarrow$ & \cellcolor{yellow!25}0.41 & \cellcolor{orange!25}\textbf{0.13} & 0.54 & 0.56 & 0.56   \\ 
% & \FLIP$\downarrow$ &  \cellcolor{yellow!25}0.3  & \cellcolor{orange!25}\textbf{0.14} & 0.42  &  0.40 &  0.43 \\ 
% & Time$\downarrow$ & 13m  & 20m & \cellcolor{yellow!25}6m  & 20m & \cellcolor{orange!25}\textbf{5m}\\ 
% & $\Delta$-loss$\uparrow$   & 2.17 & 7.58 & 1.46  & 0.08 & 0.05 \\ 
% \\
% \multirow{5}{*}{Gyroid [3D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & $6\times10^{-3}$ & 1.02& 0.15 & \cellcolor{yellow!25}$2\times10^{-3}$\\ 
% & LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.01} & 0.04 & 0.65 & 0.35 & \cellcolor{yellow!25}0.02\\ 
% & \FLIP$\downarrow$ &  \cellcolor{orange!25}\textbf{0.01}  & 0.05 &  0.61 &  0.42 &  \cellcolor{yellow!25}0.03 \\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{22.7s} & 20m & \cellcolor{yellow!25}7m & 14m & 20m\\ 
% & $\Delta$-loss$\uparrow$   & 18.2 & 18.88 & 0.72& 1.64 & 4.66 \\ 
% \\
% \multirow{5}{*}{Spheres [2D]} & Val. Error$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}$\mathbf{1\times10^{-5}}$ & 1.01 & 1.01\\ 
% & LPIPS$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{0.00} & 0.53 & 0.53\\ 
% & \FLIP$\downarrow$ &  \sout{N/A}& \sout{N/A} & \cellcolor{orange!25}$\mathbf{3\times10^{-7}}$  &  0.55 & 0.55 \\ 
% & time$\downarrow$ &\sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{4m}  & 20m & 5m\\ 
% & $\epsilon$-loss$\uparrow$  & \sout{N/A} &\sout{N/A} & 11.34  & 0.63 & 0.61 \\ 
% \\
% \multirow{5}{*}{Gyroid [5D]} & Val. Error$\downarrow$ & 0.66 & 0.65 & \cellcolor{orange!25}\textbf{$\mathbf{3\times10^{-4}}$} & \cellcolor{yellow!25}0.03 & 0.44 \\ 
% & LPIPS$\downarrow$ & 0.42 & 0.57 & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.21 & 0.54 \\ 
% & \FLIP$\downarrow$ &  0.42  & 0.62 &  \cellcolor{orange!25}\textbf{$\mathbf{6\times10^{-3}}$}  &  \cellcolor{yellow!25}0.28 &  0.60\\ 
% & Time$\downarrow$ & \cellcolor{orange!25}\textbf{2m} & 15m & \cellcolor{yellow!25}11m  & 20m & 15m \\ 
% & $\Delta$-loss$\uparrow$  & 1.92 & 1.75 & 20.34  & 2.14 & 1.60\\ 
% \\
% \multirow{5}{*}{Porous [28D]} & Val. Error$\downarrow$ & \sout{N/A} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00}\\ 
% & LPIPS$\downarrow$ & \sout{N/A} & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{orange!25}\textbf{0.61}\\ 
% & \FLIP$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{0.51} & \cellcolor{yellow!25}0.52 & \cellcolor{yellow!25}0.52 & 0.59\\ 
% & Time$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{4m} & \cellcolor{yellow!25}8m & 20m & 20m\\ 
% & $\Delta$-loss$\uparrow$  & \sout{N/A} & 0.88 & 0.01 & 1.6 & 0.23\\ 
% \end{tabular}
% \end{adjustbox}
% \caption{Reconstruction error table for different optimization algorithms (columns) and synthetic procedural structures (rows). We report for each structure the \textbf{a)} Validaton Error~\ref{validation_error}, \textbf{b)} LPIPS Perceptual loss, \textbf{c)} \FLIP error, \textbf{d)} Time of the optimization, \textbf{e)} The difference between the loss at the beginning and at the end of the optimization process denoted as $\Delta$-loss. We consider a numerical~0 to be a number below $1\times10^{-7}$. The \sout{N/A} implies that the optimization method could not be applied for the corresponding structure. }
% \label{optimization_table_results}
% \end{table}

\definecolor{darkorange}{RGB}{255,140,0}  % RGB values for dark orange
\begin{table}[ht]
\begin{adjustbox}{max width=\textwidth, max height=0.17\textheight, center}
\begin{tabular}{l r | c c c c c} 
Microstructure & Metrics & SHGO-SDF & BH-SDF & CMA-ES-SDF & CMA-ES-S & Powell-S\\
\toprule
    \multirow{4}{*}{Gyroid [1D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & \cellcolor{orange!25}$\mathbf{0.00}$ & $10^{-4}$ & \cellcolor{yellow!25}$10^{-6}$\\ 
& LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{orange!25}\textbf{0.00}& \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.02 & \cellcolor{orange!25}\textbf{0.00}\\ 
& \FLIP$\downarrow$ &  \cellcolor{yellow!25}$3\times10^{-7}$  & \cellcolor{orange!25}$\mathbf{1\times10^{-7}}$ &  $1\times10^{-3}$  &  $2\times10^{-3}$ &  $2\times10^{-3}$\\ 
& Time$\downarrow$ & \cellcolor{orange!25}\textbf{2.85s}  & \cellcolor{yellow!25}16.67s & \cellcolor{orange!25}\textbf{2.23s}  & 20m & 7m\\ 
\\
\multirow{4}{*}{Fibers [2D]} & Val. Error$\downarrow$ & \cellcolor{yellow!25}0.34 & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & 0.65 & 1.00 & 1.00\\ 
& LPIPS$\downarrow$ & \cellcolor{yellow!25}0.41 & \cellcolor{orange!25}\textbf{0.13} & 0.54 & 0.56 & 0.56   \\ 
& \FLIP$\downarrow$ &  \cellcolor{yellow!25}0.3  & \cellcolor{orange!25}\textbf{0.14} & 0.42  &  0.40 &  0.43 \\ 
& Time$\downarrow$ & 13m  & 20m & \cellcolor{yellow!25}6m  & 20m & \cellcolor{orange!25}\textbf{5m}\\ 
\\
\multirow{4}{*}{Gyroid [3D]} & Val. Error$\downarrow$ & \cellcolor{orange!25}$\mathbf{1\times10^{-3}}$ & $6\times10^{-3}$ & 1.02& 0.15 & \cellcolor{yellow!25}$2\times10^{-3}$\\ 
& LPIPS$\downarrow$ & \cellcolor{orange!25}\textbf{0.01} & 0.04 & 0.65 & 0.35 & \cellcolor{yellow!25}0.02\\ 
& \FLIP$\downarrow$ &  \cellcolor{orange!25}\textbf{0.01}  & 0.05 &  0.61 &  0.42 &  \cellcolor{yellow!25}0.03 \\ 
& Time$\downarrow$ & \cellcolor{orange!25}\textbf{22.7s} & 20m & \cellcolor{yellow!25}7m & 14m & 20m\\ 
\\
\multirow{4}{*}{Spheres [2D]} & Val. Error$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}$\mathbf{1\times10^{-5}}$ & 1.01 & 1.01\\ 
& LPIPS$\downarrow$ & \sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{0.00} & 0.53 & 0.53\\ 
& \FLIP$\downarrow$ &  \sout{N/A}& \sout{N/A} & \cellcolor{orange!25}$\mathbf{3\times10^{-7}}$  &  0.55 & 0.55 \\ 
& time$\downarrow$ &\sout{N/A} & \sout{N/A} & \cellcolor{orange!25}\textbf{4m}  & 20m & 5m\\ 
\\
\multirow{4}{*}{Gyroid [5D]} & Val. Error$\downarrow$ & 0.66 & 0.65 & \cellcolor{orange!25}\textbf{$\mathbf{3\times10^{-4}}$} & \cellcolor{yellow!25}0.03 & 0.44 \\ 
& LPIPS$\downarrow$ & 0.42 & 0.57 & \cellcolor{orange!25}\textbf{0.00} & \cellcolor{yellow!25}0.21 & 0.54 \\ 
& \FLIP$\downarrow$ &  0.42  & 0.62 &  \cellcolor{orange!25}\textbf{$\mathbf{6\times10^{-3}}$}  &  \cellcolor{yellow!25}0.28 &  0.60\\ 
& Time$\downarrow$ & \cellcolor{orange!25}\textbf{2m} & 15m & \cellcolor{yellow!25}11m  & 20m & 15m \\ 
\\
\multirow{4}{*}{Porous [28D]} & Val. Error$\downarrow$ & \sout{N/A} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00} & \cellcolor{orange!25}\textbf{1.00}\\ 
& LPIPS$\downarrow$ & \sout{N/A} & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{yellow!25}0.64 & \cellcolor{orange!25}\textbf{0.61}\\ 
& \FLIP$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{0.51} & \cellcolor{yellow!25}0.52 & \cellcolor{yellow!25}0.52 & 0.59\\ 
& Time$\downarrow$ &  \sout{N/A} & \cellcolor{orange!25}\textbf{4m} & \cellcolor{yellow!25}8m & 20m & 20m\\ 
\end{tabular}
\end{adjustbox}
\caption{Reconstruction performance for different optimization algorithms (columns) and synthetic procedural microstructures (rows). We report for each microstructure the \textbf{a)} Validaton Error, \textbf{b)} LPIPS Perceptual loss, \textbf{c)} \FLIP error, \textbf{d)} Time of the optimization. We consider a numerical~0 to be a number below $1\times10^{-7}$. The \sout{N/A} implies that the optimization method could not be applied for the corresponding microstructure. The best results are
highlighted in orange, while the second-best results are marked in yellow. }
\label{optimization_table_results}
\end{table}

\begin{figure}[ht]
    \begin{adjustbox}{max width=\linewidth, max height=\textheight}
    \setlength{\tabcolsep}{0.5pt} % Adjust column separation
    \begin{tabular}{c c c c c c c}
        & \tiny Reference & \tiny SHGO-SDF & \tiny BH-SDF & \tiny CMA-ES-SDF & \tiny CMA-ES-S & \tiny Powell-S \\ 
         \multirow{2}{*}{{\rotatebox{90}{ \tiny Gyroid [1D]}}} & \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-0_resized.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-SHGO_0_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-BH_0_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES_0_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_0.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-Powell-S_0.png} 
        \\ 
        & \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/SHGO_0.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/BH_0.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_0.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/Powell-S_0.png} \\ 
         \multirow{2}{*}{{\rotatebox{90}{ \tiny Fibers [2D]}}} & \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-1_resized.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-SHGO_1_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-BH_1_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES_1.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_1.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-Powell-S_1.png} 
        \\ 
        & \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/SHGO_1.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/BH_1.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_1.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_1.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/Powell-S_1.png} \\
        \multirow{2}{*}{{\rotatebox{90}{ \tiny Gyroid [3D]}}} & \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-2_resized.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-SHGO_2_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-BH_2_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES_2.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_2.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-Powell-S_2.png} 
        \\ 
        & \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/SHGO_2.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/BH_2.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_2.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_2.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/Powell-S_2.png} \\
        \multirow{2}{*}{{\rotatebox{90}{ \tiny Spheres [2D]}}} & \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-3_resized.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/not_applicable_rescaled.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/not_applicable_rescaled.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES_3.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_3_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-Powell-S_3.png} 
        \\ 
        & \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/not_applicable_rescaled.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/not_applicable_rescaled.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_3.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_3.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/Powell-S_3.png}
        \\
         \multirow{2}{*}{{\rotatebox{90}{ \tiny Gyroid [5D]}}} & \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-4_resized.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-SHGO_4.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-BH_4.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES_4_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_4_resized.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-Powell-S_4.png} 
        \\ 
        & \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/SHGO_4.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/BH_4.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_4.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_4.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/Powell-S_4.png}
        \\
        \multirow{2}{*}{{\rotatebox{90}{ \tiny Porous [28D]}}} & \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render-5.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/not_applicable_rescaled.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render_5_BH.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render_5_CMA_ES.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render_5_CMA_ES_S.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/fitting_render_5_Powell.png} 
        \\ 
        & \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} & 
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/not_applicable_rescaled.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/porous28d_BH.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/porous28d_CMA_ES.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/porous28d_CMA_ES_S.png} &
        \includegraphics[width=0.08\textwidth]{figures/optimization_results/errors_flip/porous28d_Powell.png}
    \end{tabular}
    \end{adjustbox}
    \caption{Reconstruction results for different optimization algorithms (columns) and synthetic procedural microstructures (rows). We show a comparison of rendered ground truth exemplars and the rendered approximations~(\textit{top row per microstructure}) with the measured \FLIP (\textit{bottom row per microstructure}).}
    \label{fig:reconstruction_renders}
\end{figure}

\clearpage
\clearpage
\begin{figure*}[ht!]
    \centering
    \begin{adjustbox}{max width=\textwidth, max height=0.5\textheight}
    \setlength{\tabcolsep}{0.5pt}
    \renewcommand{\arraystretch}{1.3}
    \arrayrulecolor{darkorange}
    \setlength{\arrayrulewidth}{0.45mm}
    \begin{tabular}{c c : c @{\hspace{0.1cm}} c : c : c @{\hspace{0.1cm}} c}
        & Reference & BH-SDF ($0.00$) & SHGO-SDF ($0.00$) & Powell ($10^{-6}$) & SIREN-VOL-512 (0.01) & SIREN-VOL-256 (0.02) \\ 
        \multirow{2}{*}{\rotatebox{90}{\centering Gyroid [1D]}} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-0_resized.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_0_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-SHGO_0_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-Powell-S_0.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/gyroid1d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/gyroid1d_siren_volume_256.png}
        \\
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_0.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/SHGO_0.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/Powell-S_0.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/gyroid1d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/gyroid1d_siren_volume_256.png}
        \\
        &  & BH-SDF ($10^{-3}$) & SHGO-SDF (0.34) & CMA-ES-S (1.00) & MLP-PE-VOL-256 (0.39) & MLP-PE-VOL-512 (0.43) \\ 
        \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{Fibers [2D]}}} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-1_resized.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_1_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-SHGO_1_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_1.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fibers2d_nerf_volume_256.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fibers2d_nerf_volume_512.png}
        \\
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_1.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/SHGO_1.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_1.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/fibers2d_nerf_volume_256.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/fibers2d_nerf_volume_512.png}
        \\
        &  & SHGO-SDF ($10^{-3}$) & BH-SDF ($6\times10^{-3}$) & Powell-S ($2\times10^{-3}$) & SIREN-VOL-512 (0.05) & MLP-PE-SUR-256 (0.06) \\ 
        \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{Gyroid [3D]}}} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-2_resized.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-SHGO_2_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_2_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-Powell-S_2.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/gyroid3d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/gyroid3d_nerf_surface_256.png}
        \\
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/SHGO_2.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_2.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/Powell-S_2.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/gyroid3d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/gyroid3d_nerf_surface_256.png}
    \end{tabular}
    \end{adjustbox}
    \caption{Renders Comparisons (\textit{continued in the next figure}). Comparison of rendered ground truth exemplars and the rendered approximations~(\textit{top row per microstructure}) with the measured \FLIP (\textit{bottom row per microstructure}). \textit{Outermost left column:}~Rendered reference. \textit{Two left columns:}~Two best analytical optimization-based methods. \textit{Middle column:}~The best analysis-by-synthesis method. \textit{Two right columns:}~Two best neural-based methods. The best methods in each section are selected based on the validation error. Based on our results show that neural networks are struggling to learn the volumetric microgeometry from SDF exemplars compared to the other two types of methods. Further exploration is needed in neural network-based experiments.}
    \label{tab:comparison}
\end{figure*}

\clearpage

% === Next part of figure ===
\begin{figure*}[ht!]
    \centering
    \begin{adjustbox}{max width=\textwidth, max height=0.5\textheight}
    \setlength{\tabcolsep}{0.5pt}
    \renewcommand{\arraystretch}{1.3}
    \arrayrulecolor{darkorange}
    \setlength{\arrayrulewidth}{0.45mm}
    \begin{tabular}{c c : c c : c : c @{\hspace{0.1cm}} c}
        & Reference & CMA-ES-SDF ($10^{-5}$) & CMA-ES-S (1.01) & Powell-S (1.01) & SIREN-VOL-512 (0.36) & SIREN-VOL-256 (0.46) \\ 
        \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{Spheres [2D]}}} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-3_resized.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES_3_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES-S_3.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-Powell-S_3.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/spheres2d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/spheres2d_siren_volume_256.png}
        \\
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_3.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_3.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/Powell-S_3.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/spheres2d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/spheres2d_siren_volume_256.png}
        \\
        &  & CMA-ES-SDF ($3\times10^{-4}$) & BH-SDF (0.65) & CMA-ES-S (0.03) & SIREN-VOL-256 (0.03) & SIREN-VOL-512 (0.04) \\ 
        \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{Gyroid [5D]}}} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-4_resized.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES_4_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-BH_4.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-CMA-ES_4_resized.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/gyroid5d_siren_volume_256.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/gyroid5d_siren_volume_256.png}
        \\
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_4.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/BH_4.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES-S_4.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/gyroid5d_siren_volume_256.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/gyroid5d_siren_volume_512.png}
        \\
        &  & BH-SDF (1.00) & CMA-ES-SDF (1.00) & CMA-ES-S (1.00) & SIREN-VOL-512 (0.7) & SIREN-VOL-256 (0.79) \\ 
        \multirow{2}{*}{\raisebox{5.5ex}{\rotatebox{90}{Porous [28D]}}} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render-5.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render_5_BH.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render_5_CMA_ES.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/fitting_render_5_CMA_ES_S.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/porous28d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/porous28d_siren_volume_256.png}
        \\
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/CMA-ES_0.png} 
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_BH.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_CMA_ES.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_CMA_ES_S.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_siren_volume_512.png}
        & \includegraphics[width=0.3\textwidth]{figures/optimization_results/errors_flip/porous28d_siren_volume_256.png}
    \end{tabular}
    \end{adjustbox}
    \caption{Renders Comparisons (\textit{continuation}). Comparison of rendered ground truth exemplars and the rendered approximations~(\textit{top row per microstructure}) with the measured \FLIP (\textit{bottom row per microstructure}). \textit{Outermost left column:}~Rendered reference. \textit{Two left columns:}~Two best analytical optimization-based methods. \textit{Middle column:}~The best analysis-by-synthesis method. \textit{Two right columns:}~Two best neural-based methods. The best methods in each section are selected based on the validation error. Based on our results, neural networks are struggling to learn the volumetric microgeometry from SDF exemplars compared to the other two types of methods. Further exploration is needed in neural network-based experiments.}
    \label{tab:comparison_contd}
\end{figure*}


==> supp_sections/reconstruction.tex <==
\section{Multiscale Geometry Reconstruction}
\label{sec:optimization}

In this section, we focus on reconstructing procedural microstructures generated by our framework. We explore two modalities: SDF, potentially extracted from noisy MicroCT scans, and RGB images potentially obtained from Transmission Electron Microscopy (TEM) or Scanning Electron Microscopy (SEM) samples. For the first modality, we apply direct parameter fitting to find the parameters of our procedural microstructures with observed data. For the second, we employ analysis-by-synthesis, iteratively refining reconstructions by comparing simulated and real electron microscopy images. For more details on the optimization approaches and algorithms, we refer the reader to the supplemental material.

\subsection{Parameter Fitting}
\label{parameter_fitting_approach}

This approach formulates microstructure reconstruction as a model fitting task, where the goal is to optimize the parameters of a procedural SDF to accurately match the microstructure's SDF groundtruth. Given a set of spatial coordinates $\Omega = \{\mathbf{x} \mid \mathbf{x} \in \mathbb{R}^3\}$, a ground-truth SDF $\hat{S}:~\mathbb{R}^3 \rightarrow \mathbb{R}$ describing the surface at the point $x$, a bounded parameter space $\Phi = [a_1, b_1] \times [a_2, b_2] \times \cdots \times [a_n, b_n]$ with $n$ parameters, and a loss function $\mathcal{L}: \mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}$, the problem is defined as minimizing the discrepancy between the fitted function $f$ and the ground truth $\hat{S}$ across the domain: 
%
\begin{equation}
\min_{\boldsymbol{\phi} \in \Phi} \int_{\Omega} \mathcal{L}(f(\mathbf{x}, \boldsymbol{\phi}), \hat{S}(\mathbf{x})) d\mathbf{x}.
\label{eq:parameter_fitting}
\end{equation}
%
Procedural SDFs allow efficient extrapolation of the microstructure beyond the optimization domain without modifying the fitted function. In addition, our compact parametrized microstructures are described with a relatively low number of parameters. We propose a loss function to evaluate the discrepancies in the frequency domain using the discrete Fourier transform (DFT) to consider the periodic behavior common in many microstructures. The loss function compares the amplitude and phase spectra of the Fourier coefficients, using the logarithm of the mean squared error (MSE) as an error metric:
%
\begin{multline}
\mathcal{L}_{FT} \left( f(\Omega, \boldsymbol{\phi}), \hat{S}(\Omega) \right) =  \\
\log \biggl( \frac{1}{2N} \sum_{i=1}^{N} \Bigl( \left| A_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi}))) - A_i(\mathcal{F}(\hat{S}(\Omega))) \right|^2 + \\
\left| \theta_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi}))) - \theta_i(\mathcal{F}(\hat{S}(\Omega))) \right|^2 + \epsilon \Bigr) \biggr).
\label{FT_loss}
\end{multline}
%
For simplicity we use $\Omega$ to express a series of points, $\mathcal{F}$ being a DFT,  $A_i(\mathcal{F}(f(\Omega, \boldsymbol{\phi})))$ and $A_i(\mathcal{F}(\hat{S}(\Omega)))$ denoting the amplitudes, and \(\theta_i(f(\Omega, \boldsymbol{\phi}))\) and \(\theta_i(\hat{S}(\Omega))\) the phases of the Fourier coefficients derived from $f(\Omega, \boldsymbol{\phi})$ and $\hat{S}(\Omega)$, respectively, \(N\) representing the number of coefficients, and $\epsilon$ being a small positive value. Recall that $A_i(\mathcal{F}(x)) = |z_i| = \sqrt{\Re(z_i)^2 + \Im(z_i)^2}$, and $\theta_i(\mathcal{F}(x)) = \arctan\left(\frac{\Im(z_i)}{\Re(z_i)}\right)$, where $z_i$ is the $i$-th Fourier coefficient of $x$, and $\Re(z_i)$ and $\Im(z_i)$ are the real and imaginary parts of $z_i$, respectively. Note this equation is closely related to the spectral density function commonly used in microstructure analysis~\cite{bostanabad2018computational}. 

\subsection{Analysis by Synthesis}
\label{analysis_by_synthesis_approach}

The analysis-by-synthesis approach optimizes the SDF by iteratively rendering it using a non-differentiable pipeline and comparing the results in image space. Given a camera intrinsics $\mathbf{K} \in \mathbb{R}^{3\times 3}$ taken from a set of intrinsic matrices $\mathcal{K}$, the camera extrinsics $\mathbf{E} = [\mathbf{R} \mid \mathbf{t}] \in \mathbb{R}^{3\times 4}$  taken from a set of extrinsic matrices $\mathcal{E}$, a labeling function $\hat{S}:~\mathbb{R}^3 \rightarrow \mathbb{R}$, a bounded parameter space $\Phi = [a_1, b_1] \times [a_2, b_2] \times \cdots \times [a_n, b_n]$ with $n$ parameters, a signed distance fitting function $f: \mathbb{R}^3 \times \Phi \rightarrow \mathbb{R}$, a loss function $\mathcal{L}: \mathbb{R}^{W\times H \times 3} \times \mathbb{R}^{W\times H \times 3} \rightarrow \mathbb{R}$, with $W, H$ being width and the height respectively, a set of functions $\mathcal{A}$, and finally the rendering function $\mathcal{R}:~\mathcal{A}\times \mathcal{K} \times \mathcal{E} \rightarrow \mathbb{R}^{W\times H \times 3}$, we can express the optimization problem as follows:
%
\begin{equation}
    \min_{\boldsymbol{\phi} \in \Phi} \mathcal{L}\left( \mathcal{R}\left( f\left( \cdot, \boldsymbol{\phi}\right), \mathbf{K}, \mathbf{E}\right), \mathcal{R} ( \hat{S}\left( \cdot \right), \mathbf{K}, \mathbf{E} ) \right).
\label{analysis_by_synthesis_eq}
\end{equation}
%
$\mathcal{R}$ renders the microstructure bounded by a unit sphere from the given view with the camera parameters using the sphere-tracing algorithm~\cite{hart1996sphere} in the CUDA-based framework OptiX \cite{parker2010optix}. For the loss function, we use the two-dimensional DFT, denoted as $\mathcal{F}_{2D}$, to transform the image signal in the frequency domain for comparison:
%
\begin{align}
\mathcal{L}_{2DFT} &\left( \mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E}), \mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E}) \right) = \notag \\
&\log \biggl( \frac{1}{N} \sum_{i=1}^{N} \left| A_i\Bigl(\mathcal{F}_{2D}(\mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E})) \Bigr) - \right. \notag \\
&\quad \left. A_i \Bigl(\mathcal{F}_{2D}(\mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E})) \Bigr) \right|^2 + \epsilon \biggr),  
\label{FT_loss_image}
\end{align}
%
where $A_i\Bigl(\mathcal{F}_{2D}(\mathcal{R}(f(\cdot, \boldsymbol{\phi}), \mathbf{K}, \mathbf{E}))\Bigr) $ and $A_i\Bigl(\mathcal{F}_{2D} (\mathcal{R}(\hat{S}(\cdot), \mathbf{K}, \mathbf{E}) ) \Bigr)$ denote the amplitudes of the 2D Fourier coefficients for the rendered image and the target image, respectively. $N$ represents the total number of coefficients, and $\epsilon$ is a small positive constant. By focusing on the amplitudes of the Fourier coefficients, we capture the key periodic features of the image, which are crucial for effective global optimization of microstructures. While a multi-view optimization is possible, we opted for a single-view approach to minimize computational overhead.

%By focusing on the amplitudes of the Fourier coefficients, we capture the key periodic features of the image, which proved to be crucial for an effective global optimization in our experiments

%While a multi-view optimization is theoretically possible, we opted for a single-view optimization due to its computational overhead, as rendering multiple views would be even more time-consuming. 

\subsection{Optimization Algorithms}

Selecting a suitable optimization algorithm is critical for solving unconstraint global optimization problems. The loss used in parameter fitting Eq. \ref{FT_loss} is differentiable allowing us to use gradient-based optimization algorithms as the operations involved are differentiable including the DFT. In this paper, we consider two first-orded methods taking advantage of the gradient information: Basin-Hoppin(BH)~\cite{wales2003energy} and Simplicial Homology Global Optimization (SHGO)\cite{endres2018simplicial} algorithms. BH algorithm is particularly effective for problems with funnel-like loss functions. Its key hyperparameters include the step size $s$ and the temperature $T$, which defines the bounds of the uniformly distributed random perturbations and the acceptance probability for the candidate function respectively. SHGO global optimization algorithm approximates locally convex subdomains using homology groups. The main hyperparameters for SHGO include the number of iterations  $l$ and the number of samples $m$ for building the complex.\\

% We can skip internal details about the optimization algorithms for the main paper.
% We can also skip internal behavior from these algorithms
% BH: Additionally, the Sequential Least Squares Quadratic Programming (SLSQP) algorithm is used as a local minimizer in the second phase, which iteratively solves a QP subproblem derived from a second-order Taylor expansion of the loss function
% SHGO: the Sobol sampling method and SLSQP are used for local search.
%
As previously mentioned, the losses functions are differentiable, but certain procedural SDFs and the rendering function $\mathcal{R}$ are non-differentiable, leading leading to non-differentiability of the final composite function. We consider two gradient-free optimization algorithms: Covariance Matrix Adaptation Evolutionary Strategy (CMA-ES) algorithm~\cite{hansen2019pycma} and modified Powell method~\cite{press1988numerical, powell1964efficient}. The CMA-ES algorithm is highly effective, in particular for rugged, noisy and non-differentiable problems. Its key hyperparameters are the population size $\mathcal{P}$ and and the initial $\sigma_0$ of the covariance matrix, typically chosen depending on the complexity and dimensional of the problem. The modified Powell method \cite{press1988numerical, powell1964efficient} is a local optimizer without hyperparameters that can be effective when a reasonably close initialization is provided.\\

==> supp_sections/related_work.tex <==
\section{Related Work} \label{sec:related}

A particulate material can be represented by distributing particles across various points in a given space. These points can be utilized to influence the coloration of textures near each point~\cite{schachter1979random}, to render the particles as images~\cite{van1991spot,dischler2002texture}, or to connect the particles into a cohesive implicit surface~\cite{ricci1973constructive}. This approach results in a volume that captures the microgeometry of the particulate material. In the following sections, we will explore related research on modeling particulate materials, with an emphasis on procedural methods for defining implicit surfaces.

\subsection{Procedural Modeling of Particulate Materials}


Modeling particulate materials often involves procedural color variation. The bombing method~\cite{schachter1979random} distributes color bubbles, later adapted for 3D textures by Peachey~\cite{peachey1985solid}, storing bubble properties in a table for efficient lookup. This eliminates the need for surface parametrization in 2D textures.

Sparse convolution noise~\cite{lewis1984texture,lewis1989algorithms} translates point distributions into particulate color variations using a convolution kernel. Efficient generation methods for kernels with compact support~\cite{frisvad2007fast,luongo2020microstructure} employ space-filling arrangements of randomly positioned impulses, simplifying neighbor identification. We use this approach to create a space-filling particle distribution within a bounding sphere radius. Sparse convolution with Gabor noise kernels~\cite{lagae2009procedural} can be used to generate high-quality surface-level textures that are spectrally controlled. In this framework, we efficiently generate high-quality volumetric hypertextures using space-filling implicit object distributions.  Stolte~\cite{1003534} presented a method for efficiently filling space and voxelizing infinite implicit objects using recursive subdivision algorithms, which work best for repetitive structures and capture intricate details, such as cyclical surfaces.

Hypertexture~\cite{perlin1989hypertexture} extends color variation to density variations in a volume, enabling procedural surface rendering via ray marching~\cite{tuy1984direct,kajiya1984ray}. Worley~\cite{worley1996cellular} demonstrated that distances to nearest points effectively model surface irregularities in particulate materials. We apply this to transform our particle distribution into an SDF for physically based rendering.

Stereology estimates 3D particle number density from 2D exemplars, aiding tileable color variation in particulate materials~\cite{jagnow2004stereological,shu2014efficient}. The Worley method~\cite{dorsey1999modeling,soulie2007modeling} generates compact particle aggregates using a precomputed Poisson point distribution. Randomized particle instantiation within a volumetric tile disrupts tiling periodicity~\cite{meng2015multi}, while space-filling point distributions eliminate the need for tiling or precomputation~\cite{baerentzen2023curl}. We leverage this to create spatially variable particulate materials with an SDF representation.

Radial basis functions can encode color and SDF from 2D reference images~\cite{qian2023vector}. Unlike these localized precomputed variations, our approach provides functional shape modeling tools that operate throughout space, maintaining a fully space-filling SDF.

\subsection{Signed Distance Field Modeling and Rendering} 
Ricci~\cite{ricci1973constructive} defines solid surfaces using level sets within a distance field, employing $\max$ and $\min$ for union and intersection. Hart et al.\cite{hart1989ray} optimized rendering for such implicit objects, leading to sphere tracing\cite{hart1993sphere, hart1996sphere}, now widely used for rendering SDF-based objects. We leverage sphere tracing for Monte Carlo ray tracing of microgeometries.

Function-based representation of objects, along with the relations and operations defined by Pasko~\cite{pasko1995function}, has been used for blending, offsetting, and morphing geometric shapes and objects. SDFs enable Boolean operations, surface offsets, and blending via interpolation~\cite{payne1992distance}. Our particulate SDF modeling integrates these methods with spatially varying offsets. While SDFs can also model layered solids~\cite{cutler2002procedural}.

Precomputed SDFs benefit from adaptive grids for scalability~\cite{frisken2000adaptively}. Sparse voxel octrees improve multi-scale representation and interpolation~\cite{heitz2012representing}, while displacement fields reduce voxelization artifacts~\cite{brunton2021displaced}. Our procedural approach avoids voxelization artifacts and precomputation constraints, ensuring smooth scale transitions, though high sample counts are needed for antialiased rendering. Adaptive ray marching~\cite{morrical2019efficient, wu2022real} improves the efficiency of the sphere tracing method. We extend it to multiscale geometry modeling with adaptive grids, where varying grid scales in different volume regions require adaptive bounds (or stepping) for better performance than fixed-length steps. We used longer steps in coarse grid resolution and shorter steps in fine grid resolution adaptively.

ShaderToy provides procedural SDF modeling resources~\cite{jeremias2014shadertoy} (\href{https://www.shadertoy.com/}{https://www.shadertoy.com/}), while Takikawa et al.~\cite{takikawa2022dataset} offer optimized SDF functions. In our work, an SDF-defined macroscopic surface influences the size, shape, and density of contained particles.



\subsection{Simulation-based Particulate Materials}
Particle simulation offers an alternative to point distribution for generating particulate materials. Discrete element methods simulate particle motion and interactions~\cite{bell2005particle,zingsheim2024learning}, even for arbitrarily shaped particles using SDFs~\cite{lai2022signed}. However, managing large particle counts efficiently remains a challenge. Our on-the-fly particle generation can overcome this. Continuum-based modeling~\cite{narain2010free} could enable consistent particulate generation within a medium, presenting an interesting future direction.

Other physically-based simulations~\cite{zhao2023role} produce realistic particulate materials, such as in bread-making~\cite{baravalle2015procedural}, but require substantial pre-computation, memory, and resolution constraints.

Additionally, other physically-based simulation techniques can yield impressive results in particulate materials~\cite{zhao2023role}, such as in simulations of bread-making~\cite{baravalle2015procedural}. However, these methods often demand substantial pre-computation and memory usage, along with constraints regarding material extent and resolution.

\subsection{Neural-based Techniques}

Perlin noise~\cite{perlin1985image,perlin2002improving} combined with an encoder-decoder neural network can generate realistic 3D textures from 2D references~\cite{henzler2020learning}. Implicit periodic field networks use periodic encoding in MLPs to model particulate materials~\cite{chen2022exemplar}, but their reliance on precomputed 3D subvolumes makes them impractical for large-scale rendering.

A volumetric shell approach with material texture patches~\cite{kajiya1989rendering} can be enhanced using neural techniques~\cite{baatz2022nerf,kuznetsov2022rendering,diolatzis2023mesogan,huang2023nerf}. Unlike these methods, we provide an exact mesoscale geometry representation, which is essential for applications like transparent particles (e.g., air bubbles in ice). Generative models for spatially varying noise~\cite{maesumi2024one} are limited to surface noise, while learning volumetric noise remains challenging. Our work explores SDF-based volume reconstruction, enabling full-volume reconstruction from examples.

\subsection{Miscellaneous Methods}

 Hypervolume model~\cite{pasko2001constructive} explores volume representation using functional representations (FRep) with attributes, generating hypervolumes via constructive tree structures and blending operations. Inspired by the hypertexture mechanism, we developed a framework that dynamically generates spatially varying microstructures using implicit functions and CSG operations.

Volume perturbations~\cite{kniss2002interactive} capture high-frequency details for realistic material appearance, while generalized displacement maps~\cite{wang2004generalized} render non-height-field mesoscale structures. We employ perturbations to enhance microgeometry details in volume rendering.

Periodic surface modeling~\cite{wang2007periodic,lu2022structural} with triply periodic minimal surfaces (TPMS) enables intricate topological patterns across scales, including composite metamaterials. Leveraging trigonometric functions, we generate seamless multiscale microstructures with minimal parameters and computation.

Geometry textures~\cite{toledo2008geometry} and volumetric spot noise~\cite{turkay2016volumetric} synthesize surface details but are limited to surfaces. MesoGen~\cite{michel2023mesogen} tiles mesoscale patterns aperiodically on meshes. Unlike these, our framework uses implicit functions to generate spatially varying infinite microstructures inside volumes.

Porous material modeling~\cite{baravalle2017realistic} employs particle systems and procedural Voronoi foams~\cite{martinez2016procedural} for additive manufacturing but is restricted to porous structures. Point distributions~\cite{sahbaei2018implicit,baerentzen2023curl} create convex, blob-like porous microstructures but lack spatial variation. We introduce agglomeration to generate complex, curvy, laminar, and fibrous microstructures, enabling mixed media, multiscale properties, and regionally varied packing densities.

==> supp_sections/rendering.tex <==
\section{Multiscale Geometry Rendering} \label{sec:st}

We use conventional ray tracing methods when we render particulate geometry bounded by a triangle mesh. The sign of particulate material SDF \( d_g \) at the surface indicates whether the ray interacts with the particles' material or the host medium. Our approach focuses on the surfaces of light-scattering many particles, giving the flexibility to use only surface shaders along with volume absorption~\cite{pharr2023physically}. One important aspect is that this choice is not a limitation of our method, but it highlights our capability to model particle geometry and render light scattering volumes using straightforward surface shaders.

We need to find the next surface intersection when once the path is in mesoscale geometry; we start by storing the sign of the first SDF and apply a minimum distance to prevent locating the ray's origin as the intersection point. Following the methodology of Hart's sphere tracing~\cite{hart1996sphere}, we proceed along the ray by utilizing the value of $d_g$ multiplied by the initial sign, which facilitates tracing through transparent particles. The normal vector is then employed for surface shading at a surface intersection point; we calculate the gradient of the SDF using central differences.

To terminate paths probabilistically, we implement a Russian roulette technique that is based on absorption occurring at a diffuse particle surface or through volume absorption between surfaces. Additionally, we establish a maximum trace depth, at which point we return black if it is exceeded. When determining the maximum trace depth for a scene, we start with an initial rendering with a low value of the maximum trace depth. This approach can result in the rendered material appearing darker due to early path termination. We then incrementally raise the maximum trace depth until the brightness of the rendered material stabilizes. Figure~\ref{fig:clustersizeintensity} illustrates the trace depth for various particle clouds with distinct parameters.

%One of the main advantages of our method, as compared with statistical methods based on scattering properties, is that our simple rendering pipeline works for all types of particles, from spherical to non-spherical. If we compute scattering properties using Lorenz-Mie theory, the distribution of the scattered light is only accurate for spherical particles. Computing scattering properties for non-spherical particles is a complicated task.

In general, we divide 
$d_g$ by the greatest magnitude of the gradient to ensure that the functions represent signed distance despite potentially being transformed to a non-Euclidean domain. We list some rules that we follow when performing affine transformations on point a $\bm{p}$ in the supplemental material for various Lipschitz bounds used for the affine transformations.

==> supp_sections/suspended_particulate_media.tex <==
\section{Discrete Grid-based Geometry Modeling}

A SDF is a scalar field that provides the minimum distance from a point \(\bm{p}\) to the surface defined by an implicit function. It is negative when the point is inside the surface, positive when outside, and zero when it lies on the isosurface~\cite{frisken2000adaptively}.

This section covers the principles for synthesizing various geometric patterns using discretized grid SDFs using space-filling primitives. Sec.~\ref{sec:spm} covers the modeling of suspended particulate media through space-filling primitive SDFs. Sec.~\ref{sec:pa} covers modeling various geometric patterns through particle agglomeration. Sec.~\ref{sec:pp} covers modeling the granular media through particle piling. We focus on filling a specified volume with primitives through implicitly defined primitive geometry. Several implicit functions with methods and operations are useful for generating hypertextures for real-world microstructures. As a general case, we start with spherical primitives as particulate geometry. We can find the nearest overlapping particulate structures by evaluating a function at any spatial point denoted as $\bm{p}$. To facilitate the rendering of this geometry, we employ surfaces such as triangle meshes to outline regions in a three-dimensional space. In the following sections, we will explain our method for modeling particulate geometry for various types, including particle suspensions, particle agglomerations, and particle piling.

\subsection{Modeling Suspended Particulate Media} \label{sec:spm}
Suspended particulate media consist of discrete particles in 3D space with no contact between them. In this section, we introduce the dual-grid-based approach for generating suspended particulate media, along with various principles for creating spatially varying particulate media with variations in density, distribution, shape, size, correlations, anisotropy, noise particles and more.



\subsubsection{Point Distribution with Random Instantiation} \label{sec:pointdistrib}

To generate particulate microgeometry, we require a space-filling point distribution that facilitates random instantiation of particles and provides a straightforward method to find any nearest particles that might overlap with a given point in space $\bm{p}$. Taking inspiration from methods used to produce sparse convolution noise~\cite{frisvad2007fast,luongo2020microstructure}, we accomplish this by utilizing a regular cubic grid in conjunction with a seeded pseudo-random number generator (PRNG). The grid cell index $\bm{q} = (q_x, q_y, q_z)$ is incorporated into a multilinear spatial hash function and then multiplied by the number of random numbers needed for a cell, denoted as $N$, to create a seed $t$ for the PRNG. By setting $N = 4$, we can generate a particle of random size $s$ and position $\bm{x}$ within each grid cell:

\begin{eqnarray}
t & = & N \sum_{i=0}^1\sum_{j=0}^1\sum_{k=0}^1a_{ijk} q_x^i q_y^j q_z^k \label{eq:seed}\\
(\xi_1,\dots,\xi_N) & = & \mathrm{rnd}(t, N) \label{eq:rnd}\\
\left[\bm{x}, s\right] & = & [\bm{q} + (\xi_1, \xi_2, \xi_3), \xi_4] \,, \label{eq:instance}
\end{eqnarray}
The pseudorandom number generator (PRNG), denoted as $\mathrm{rnd}$, produces $N$ random numbers that are uniformly distributed within the interval $[0,1)$. The coefficients $a_{ijk}$ are chosen to remove regularity artifacts in the distribution of particles that result in the process of generating particle clouds. Choosing prime numbers as coefficients eliminates the regularity artifacts in a better way.

To accurately identify particles that might overlap with a point \(\bm{p}\), we control the radius of the particle's bounding sphere to no more than half the width \(w\) of a grid cell. As a result, we can calculate the indices of the eight grid cells that could potentially contain particles overlapping the point \(\bm{p}\).
\begin{eqnarray}
\bm{q}_i & = & \left\lfloor\bm{p}_w - \left(\frac{1}{2}, \frac{1}{2}, \frac{1}{2}\right)\right\rfloor \nonumber\\
& & {}+\left(i\!\!\!\!\mod 2, \left\lfloor\frac{i}{2}\right\rfloor\!\!\!\!\!\mod 2, \left\lfloor\frac{i}{4}\right\rfloor\!\!\!\!\!\mod 2\right) \nonumber\\
& & \text{for $i = 0,1,\dots,7$,} 
\label{eq:cellid}
\end{eqnarray}
%where $\bm{p}_w = \frac{1}{w}(\bm{p} + \bm{h}(\bm{p}))$ scales the coordinates according to the grid cell width and accounts for domain warping by an arbitrary vector function $\bm{h}$.
%The subtraction by $\frac{1}{2}$ from each scaled coordinate and flooring corresponds to using a dual grid with a half-cell width offset so that a point $\bm{p}$ in a cell of the dual grid can only be influenced by particles in the $2^D$ surrounding cells, where $D$ is the number of dimensions (see Figure~\ref{fig:distrib}).

The expression \(\bm{p}_w = \frac{1}{w}(\bm{p} + \bm{h}(\bm{p}))\) scales the coordinates based on the width of the grid cell and incorporates domain warping through an arbitrary vector function \(\bm{h}\). The adjustment of subtracting \(\frac{1}{2}\) from each scaled coordinate, followed by flooring, effectively utilizes a dual grid with a half-cell width offset. This design ensures that a point \(\bm{p}\) located within a cell of the dual grid is influenced solely by particles in the \(2^D\) neighboring cells, where \(D\) represents the number of dimensions (refer to Figure~\ref{fig:distrib}).

\begin{figure}
\centering
\begin{tabular}{@{}c@{}c@{}}
 \includegraphics[width=0.5\linewidth, height=9.5em]{images/dual-grid2}\hspace{\stretch{1}} &
\includegraphics[width=0.5\linewidth, height=9.5em]{images/dual-grid-3d} \\[-0.5ex]
    \end{tabular}
\caption{To consider the particles that may overlap an arbitrary query point $\bm{p}$, we check that the bounding sphere radius of a particle is at most half a grid cell width. Once we identify the cell in the stippled dual grid to which $\bm{p}$ belongs, the particles that could potentially overlap must be found in the $2^D$ grid cells that intersect with the stippled dual-grid cell (where $D$ represents the number of dimensions).}
\label{fig:distrib}
\end{figure}

Our method of using a bounding sphere for particles within a grid cell ensures that we capture all relevant particles near our point of interest, \(\bm{p}\). Still, we face a slight challenge because we can only interact with the particles in the eight neighboring grid cells. While it's true that particles in farther grid cells won’t overlap with \(\bm{p}\), one of them might actually have the closest surface. To navigate this, we set a limit on our SDF to half the grid cell's width, ensuring we don't cross the bounding sphere of the nearest particle during sphere tracing. This method might lead us to inadvertently move into a particle, resulting in a negative SDF value that is not visible in the neighboring cells. In such cases, our tracing process will need to backtrack a bit to find the surface that we initially missed. Fortunately, this scenario is easily determined by noticing a change in sign in the SDF value on our next step along the ray. This allows us to refine our tracing method, making the process more effective and reliable.

\subsubsection{Particle SDF in a Grid Cell} \label{sec:particle}

%We can use any particle shape within a grid cell as long as its bounding sphere radius is at most $w/2$. This means our method is unsuitable for fibrous materials but well-suited for particulate materials. The simplest SDF is, of course, that of the sphere. Suppose $[\bm{x},s]$ denotes the random instantiation of the particle in the grid cell of index $\bm{q}$, as described in Eq.~\ref{eq:instance}, we let $d_{\bm{q}}$ denote the signed distance function describing this particle. For a randomly placed sphere of random radius between $0$ and $w/2$, we have

Any particle shape can be used within a grid cell as long as its radius of the bounding sphere does not exceed \( w/2 \). The simplest SDF is that of a sphere. However, we could use any kind of particulate shape, see Fig.~\ref{fig:rbc} for particle shape as a red blood cell (RBC). Let \( [\bm{x}, s] \) represent the random placement of the particle within the grid cell indexed by \( \bm{q} \), as outlined in Eq.~\ref{eq:instance}. We denote \( d_{\bm{q}} \) as the signed distance function that describes this particle. For a sphere that is randomly placed with a radius that varies between \( 0 \) and \( w/2 \), we have
\begin{equation}
d_{\bm{q}}(\bm{p}_w) = \|\bm{p}_w - \bm{x}\| - \frac{1}{2}s \,.
\label{eq:p-sdf}
\end{equation}
To make things easier, we make the function accept a scaled point of interest as an argument, enabling the particle's signed distance function to be defined in a 3D space where the grid cell width is 1.

We can easily control the center of the particle at \(\bm{x}\) to a smaller portion of the grid cell or constrain its radius to a narrower range of values. By adjusting \(N\) in Eqs.~\ref{eq:seed}--\ref{eq:rnd}, we can define the particle using fewer or more random numbers. For example, we might set a fixed radius for all particles (\(N=3\)), or we could employ two random numbers to achieve random orientations of fixed-size ellipsoids (\(N=5\)). Spherical particles often serve as an excellent foundation for generating various particle shapes, while ellipsoids can be created through directional scaling, see Fig.~\ref{fig:anisotopic_ice}. As mentioned in Sec.~\ref{sec:related}, there are many SDFs of different shapes available in the literature and online. Furthermore, we can utilize Boolean operations to merge various particle clouds with different shapes together. Many SDFs applied in practice are non-Euclidean, such as those ellipsoids generated by directional scaling. Consequently, the step length in sphere tracing must be adjusted by multiplying it by the reciprocal of the Lipschitz bound of the implicit surface function~\cite{hart1996sphere}. In this context, the Lipschitz bound refers to the maximum magnitude of the gradient of the SDF.




\subsubsection{Particulate Material SDF and Spatial Variation} \label{sec:particulate}

We now introduce the SDF for the particle suspensions. In this context, the subscript \(i\) refers to one of the eight nearest grid cell neighbors, indicated by the index \(\bm{q}_i\), as outlined in Eq.~\ref{eq:cellid}. The SDF for the suspended particulate material is then defined as follows:
\begin{equation}
d_g(\bm{p}, w) = f(\bm{p}) + \min_{i=0,\dots,7} d_{\bm{q}_i}\left(\frac{1}{w}(\bm{p} + \bm{h}(\bm{p}))\right) \,, \label{eq:g-sdf}
\end{equation}
where $f$ is an arbitrary function for spatially varying offsetting of the surface.
%and $\bm{h}$ is an arbitrary vector function for domain warping. 


The amount of frequency of the function $f$, can introduce noise to the surfaces of the particles or influence their sizes in various spatial regions. Besides $f$, we also utilize the grid cell width $w$ and impose limits on the particle size $s$ to manage the number density and size distributions of the particles. Additionally, constraints on $\bm{x}$ can be applied to regulate the balance between regularity and randomness in the point distributions for positioning the particles within the cloud.
%Figure~\ref{fig:svb} shows the modeled particle cloud with all those functionalities explained in Equation~\ref{eq:g-sdf}.

The transformation of the point $\bm{p}$ using the turbulent or noise matrix can be employed to generate multi-phase particle clouds (see Fig. ~\ref{fig:ice_multiphase}) and particles with noisy or wavy patterns. Please refer to the supplemental material for more details on the multi-phase particle cloud generation.

The constraints in the above method are placed on particle sizes within a given grid; we can effectively use Boolean operations to merge various particle inclusions. For instance, by employing the minimum (or union) operator, we can integrate SDFs that exhibit unique local variations, which allows us to blend different distributions of particle sizes and densities (refer to Fig.~\ref{fig:svbunny}).

\begin{figure}[tb!]
  \includegraphics[width=\linewidth]{images/rbc_ns_closer1.png} \\[-1.5ex]
 %\includegraphics[width=0.50\linewidth]{teaser_results/food_plate.png}
    \caption{RBC particle cloud modeled using our method and an implicit function available for the shape of these cells in~\cite{kuchel2021surface}.}
  \label{fig:rbc}
\end{figure}




\subsubsection{Particle Size and Number Density Distribution Control} \label{sec:control}

%As mentioned, we can control the size and the number density distributions of a material.


To bridge the digital scene with a physical length scale, it's essential to define the physical length of a unit within the digital domain, which we denote as the scene scale~$\ell$. Consequently, the physical width of a grid cell is given by $\ell w$, resulting in a particle number density of $N = (\ell w)^{-3}$ when there is one particle per grid cell. For a specified grid cell width~$w$, the maximum radius of the bounding sphere for a particle, according to our method, is $r_{\max} = \frac{1}{2}\ell w$. Within this framework, we can choose the particle shape and scale~$s$ freely. To create a tailored particle size distribution, we produce the pseudo-random numbers required for our random instantiation (refer to Sec.~\ref{sec:pointdistrib}) and sample $s$ based on a probability density function (pdf), see Fig.~\ref{fig:validation} for the appearance of a material modeled with a normal distribution of particle sizes. A range of sampling methods (including normal distribution sampling) can be found in the work of Shirley et al.~\cite{shirley2019sampling}. This process allows us to simulate materials with specific particle size distributions. Furthermore, employing offsetting (the function $f$ detailed in Sec.~\ref{sec:particulate}) or adjusting the distribution parameters based on the location of interest $\bm{p}$ results in heterogeneous materials, where particle density varies throughout the volume.

To blend particles of various shapes, we employ random instantiation to sample a piecewise constant pdf through a method similar to Russian roulette, using predetermined probabilities for each shape. Moreover, we utilize a rejection control technique where a spatially varying function \( g(\bm{p}) \), ranging between 0 and 1, dictates the likelihood of accepting a particle within a given grid cell. In each grid cell, we apply a Russian roulette method using a random number \( \xi_j \) from our instantiation, such that if \( \xi_j < g(\bm{p}) \), the particle's SDF is represented as \( d_{\bm{q}}(\bm{p}_w) \); otherwise, it is set to \( \infty \).






\subsubsection{Particle Correlation} \label{sec:correlation}

Our approach also allows the modeling of spatial correlations among particles, a concept that is also applicable in volume path tracing without creating individual surfaces of the particles~\cite{jarabo2018radiative}. When the positions of particle centers $\bm{x}$ are fixed within the grid cells rather than being randomly initialized (as discussed in Sec.~\ref{sec:particle}), the particles are arranged in a regular cubic lattice, which is referred to as exhibiting negative spatial correlation. Conversely, if $\bm{x}$ is completely randomized within the range of $[0,1]^3$ through random instantiation, we achieve a stratified random distribution of particle locations, often described as spatially uncorrelated particles. Between these two extremes, it is also possible to create a positive correlation, where particles tend to cluster together in groups.

The rejection sampling technique is an effective tool for controlling positive correlation. Some particles can be removed to allow existing particles to form clusters. The number of clusters and the number of particles for each cluster depend on the function $g(\bm{p})$ used for rejection sampling. As an example, the modular function 
\begin{equation}
g(\bm{p}) = \left\{\begin{array}{l@{\,,\quad}l}1 & \prod_{i \in \{x, y, z\}} \left| \operatorname{mod} (|p_i|, n) \right| < \frac{n}{2} \\ 0 & \textrm{otherwise}\end{array}\right.
\end{equation}
generates positively correlated particles of 
size $(\frac{n}{2})^3$.

It is possible to modify the above equation in many ways to generate particle clusters of varying sizes and densities. Another way to generate organic particle clusters is by using multi-level particle clouds, where we first generate a particle cloud and then generate a particle cloud inside every single particle, see Fig.~\ref{fig:corr}. The following is the SDF representing particle clusters of size $n$:
\begin{equation}
d_{\text{clusters}}(\bm{p}, w) = \max(d_g(\bm{p}, 2w/n), d_g(\bm{p}, w)) \,.
\end{equation}


%All of these can be controlled by adjusting the seed for the pseudo-random number generator. Essentially, the seed is determined by a polynomial hash function of point coordinates $\bm{p}$ with a maximum degree of 4. A polynomial function of this degree with coefficients in prime numbers is sufficient for achieving randomness in distribution of particles.


\begin{figure}[tb]
 \centering
  \begin{tabular}{@{}c@{}c@{}}
   \includegraphics[width=0.5\linewidth]{images/cube_5.png} &
  \includegraphics[width=0.5\linewidth]{images/ice_small_1.jpg} 
  \\[-0.5ex]
  \end{tabular}
\caption{Inspired by a photo of air bubbles in ice (right), we used our multi-phase particle cloud approach to model a similar material (left). Our model has ice as the host medium and contains air particles that vary in size and shape with the spatial location in the medium, transitioning from spherical to non-spherical.}% \textcolor{blue}{We already talked about it, right now our zoom in pictures showing meso scale details, adding more closer versions is making a triplet like macro. meso, and micro appearance of geometric details.}}
\label{fig:ice_multiphase}
\end{figure}






\subsection{Modeling Particle Agglomeration} \label{sec:pa}

In this framework, particle agglomeration is the mechanism by which individual particles in the regular lattice grow in size and stick together to form other geometric structures. We focus on modeling particle agglomeration using the cubic regular lattice (or crystalline structure) of spherical particles. We sample clusters of particles from the regular lattice and we use a union operator (the minimum in a SDF) to combine them. We refer to this union of particles that touch as particle agglomeration. The above dual grid approach described works only for the suspended particulate media because there is a limitation on the size of the particle. For modeling the particle agglomeration, we need to consider the 27-neighborhood of the point for SDF evaluation. Also, there is no limitation on the particle size, which means particles grow in size and can stick together to form agglomerates. From this method we are able to control the crystal growth mechanism in materials. We use particle agglomeration to synthesize different types of microstructures from the regular lattice of spherical particles.

For the particle agglomeration, our starting point is a cubic regular lattice. For any point in space \(\bm{p}\), we find the index of the grid cell it occupies using \(\bm{q} = \lfloor\bm{p}/w\rfloor\), where \(w\) represents the width of the grid cell. This index can then be applied in conjunction with xor-shift bit scrambling~\cite{marsaglia2003xorshift} to generate a seed for PRNG, which may be useful for random instantiation or for controlling geometry rejection within a grid cell. We utilize the index \(\bm{q}\) to explore the 27-neighborhood of grid cells surrounding the point \(\bm{p}\). If a particle within cell \(\bm{q}\) has a radius of at most \(w\), it will not overlap with any cells beyond the 27-neighborhood.

With respect to the 27-neighbourhood of the point point \(\bm{p}\), we change the equations \ref{eq:p-sdf} and \ref{eq:g-sdf}, in the following manner for generating the particle agglomeration. We can utilize any particle shape within a grid cell as long as its bounding sphere radius satisfies \( r \leq w \). By scaling the point of interest as \( \bm{p}_w = \bm{p}/w \) and defining \( \bm{c} \) as the relative center of the sphere within the grid cell, the SDF that describes a sphere located in the grid cell indexed by \( \bm{q} \) is given by.
\begin{equation}
d_{\bm{q}}(\bm{p}_w) = \|\bm{p}_w - \bm{q} - \bm{c}\| - \frac{r}{w} \,.
\label{eq:particlesdf}
\end{equation}

Letting $\bm{q}_i$ denote the index of one of the 27 nearest grid cell neighbors surrounding a point $\bm{p}$; we evaluate the SDF using
\begin{equation}
d_g(\bm{p}, w) = f(\bm{p}) + \min_{i=0,\dots,26} d_{\bm{q}_i}\left(\frac{1}{w}(\bm{p} + \bm{h}(\bm{p}))\right) \,, \label{eq:pa-sdf}
\end{equation}

Given the restriction of $r \leq w$, particles that lie outside the 27-neighborhood cannot overlap with any point in the grid cell containing $\bm{p}$. Nevertheless, there may be particles beyond this neighborhood that are closer than what is represented by the geometry of these 27 grid cells. To control overlapping with any particle positioned in a grid cell outside the 27-neighborhood during sphere tracing, we limit $d_g$ to $w/2$.

This framework has no limitation on using non-spherical particles as the basic geometric primitive. It is entirely feasible to utilize a variety of other primitives, such as cubes, tori, cylinders, ellipsoids, hexagonal prisms, thin hexagonal prisms, etc. Essentially, the framework can adapt to any kind of geometric primitive, allowing for a wide range of microstructure modeling possibilities; for this, one could simply replace the primitive sphere in Eq.~\ref{eq:particlesdf} with another target primitive. For instance, see Figure.~\ref{fig:primitive-fibers} for fibrous microstructure generated using the space-filling of cylindrical primitives.

\begin{figure}
    \centering
    \begin{tabular}{@{}c@{}c@{}}
        \begin{tikzpicture}

  % Insert the image
  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.237435\textwidth]{images/scene_bc1.png}};

  % Define coordinates for drawing (relative to the image)
  \begin{scope}[shift={(image.south west)}, x={(image.south east)}, y={(image.north west)}]
  
    % Draw a curve on the image (Bezier curve)
    \draw[red, thick] (0.,0.43) .. controls (0.4,01.263126) and (0.6419586,0.238721) .. (0.6427,0.21);
  
    % You can add more curves, lines, or shapes as needed
  \end{scope}

\end{tikzpicture}
 \includegraphics[width=0.5\linewidth]{images/Beizer_curve_gel.png}  \\[-2ex]
 \end{tabular}
  \caption{Particle agglomeration structures generated using B{\'e}zier curves as polynomial functions on grid cell $\bm{q}$ in the 27-neighbourhood of the point $\bm{p}$. The shape of each agglomerate is different from the others. It is spatially varying throughout a large section of microgeometry. The particle arrangement mimics a snapshot of a gelation process. See Eq. 9 in the supplemental material for corresponding B{\'e}zier curves for this. }
  \label{fig:bc}
\end{figure}

\subsubsection{Particle Agglomeration through a Modular Lattice Subset}

We synthesize different types of meso- and microscopic materials based solely on spherical particle clouds arranged in regular lattices. The particulate material SDF, $d_g(\bm{p}, w)$, generates particle clouds with a regular distribution of particles of size $r$ at every grid cell. By using an integer-valued polynomial ($P$) or rational ($R$) function with the grid cell index as an argument, we can do rejection control, meaning that some particles in the regular lattice are removed, and the remaining particles stick together (if large enough) to form other shapes such as fibers, laminar structures, and porous lattices. Using a set theory approach, we select a subset of particles from the total particle population. For instance, in Figure~\ref{fig:bc}, we sample gels using B{\'e}zier curves, causing the particles to stick together in curve-like shapes. This allows us to derive an arbitrary type of microgeometry from the regular particle distribution. Moreover, we can jitter a regular particle cloud into a highly irregular particle distribution using polynomials for the rejection control.

In general, every micro- or mesoscopic structure can be defined by a particle cloud, where each particle is associated with a binary value of either zero or one. If the value is zero, the particle is removed, and if it is one, the particle is retained. For a volume of size $u \times v \times w$, this results in $2^u \times 2^v \times 2^w$ possible micro- or mesoscopic structures. Essentially, we need to find a polynomial or rational function that operates on particle clouds to generate various structures. This implies that every microstructure can be generated using a regular lattice of particle clouds, which could be useful for learning microstructures or reconstructing volumes from examples inspired by particle agglomeration mechanisms.

Suppose we let $D: \mathbb{Z}^3 \to \mathbb{B}$ be a function mapping a grid cell index $\bm{q}$ to a Boolean value. This function selects a subset of particles from the cubic regular lattice in such a way as to synthesize a microstructure. This is sufficiently general to define particulate, fibrous, laminar, porous, or mixed geometries. When the function returns true (1), the SDF of the particles is included in this part of the space. If $D$ returns false (0), we set the SDF to $w/2$. We define the non-Euclidean SDF for this type of material by
%
\begin{equation} \label{eq:sdf}
d(\bm{p}, w) = \begin{cases} 
d_g(\bm{p}, w)\,, & \text{for\ }  \bigwedge_{i=0}^{26}[D(\bm{q}_i) = 1], \\
w/2\,, & \text{otherwise},
\end{cases}
\end{equation}
where $\bm{q}_i$ are the grid cell indices of the 27-neighborhood around $\bm{p}$ and $[C]$ is an Iverson bracket returning $1$ if the condition $C$ is true and $0$ otherwise. We specify the grid cells containing geometry using
%
\begin{equation}
D(\bm{q}) = 
\begin{cases} 
1\,, & \text{if } \bigoplus_{i=1}^{k_1} \bigoplus_{j=1}^{k_2} [P_i(\bm{q}) \equiv c_{ij} m_{ij}\!\!\pmod{m_i}], \\
0\,, & \text{otherwise}.
\end{cases}
\label{eq:pf}
\end{equation}
where $P_i(\bm{q})$ are multivariate integer-valued polynomial functions, and $m_i$ with $i=1,\dots,k_1$ are positive integer moduli for the polynomials $P_i(\bm{q})$. We can also use inequalities instead of congruency in the Iverson bracket.

The symbol \(\bigoplus\) represents either the reduction operator version of logical OR ($\bigvee$) or logical AND ($\bigwedge$). The inner \(\bigoplus\) operator can be used to select different congruence classes of the same polynomial, while the outer \(\bigoplus\) operator can be used to select congruence classes across the polynomials.  %when we check the condition in.~\ref{eq: pf}, we use these logical operators, but basically, these represent  (\(\sum\)) or (\(\prod\)) between polynomials. %; even in the general case for the polynomials, it represents either (\(\prod\)) or (\(\sum\)). 
%The operator $\bm{1}_A(\bm{x})$ is the indicator function, which is 1 if $\bm{x} \in A$ and 0 otherwise.
The binary coefficients \(c_{ij}\) can be either -1 or 1 and are used to select a specific congruence class for the individual polynomials with respect to their modulo; if it is -1 then the specific congruence class is not included, and when it is 1 the congruence class can be included. The integers \(m_{ij}\) are constants such that \(0 \leq m_{ij} < m_i\), while \(m_i\) is the modulus for the \(i\)-th polynomial,  and the integers \( k_1 \) and \( k_2 \) are selected such that \( k_1 \geq 1 \) and \( k_2 \leq m_i \). 
%and \(m\) is the common modulus such that \(m = \bigoplus(m_i)\) for all \(i\). 
In some cases, a rational function could be used instead of a polynomial function in the above equation. 

\begin{figure}
    \centering
    %\includegraphics[width=0.33\linewidth]{images/cheese_tightly_loose.png}&
   \begin{tabular}{@{}c@{}c@{}}
    \includegraphics[width=0.5\linewidth]{images/fibers_sitting.png}
    \includegraphics[width=0.5\linewidth]{images/fibers_sitting1.png}
    %\includegraphics[width=0.33333\linewidth]{images/gyroid_1-25.png}
    \end{tabular}
  \caption{ Left: Fibrous microstructure with diameter 1mm generated using particle agglomeration method, right: same microstructure as left but smooth it using the smin operator. We generate the snapshot of the processes of particle agglomeration (the clustering of particles) and crystal growth using polynomial functions on the regular lattice of particle clouds. }
  \label{fig:fibers_sitting}
\end{figure}



\subsubsection{Meso-scale Surface Patterns on the Macrosurface}\label{sec:micro-macro}

Meso-scale surface patterns on macroscopic objects can be generated using the family of polynomial functions, but without doing the modular operation, this leads to selecting the subset of particles from the regular lattice based on some conditions of these polynomial functions.  This approach leads to on-the-fly generation of various macroscopic objects with spatially varying microgeometry embedded in them. The following condition explains generating the SDF for this: 
%

\begin{equation}
d(\bm{p}, w) =
\begin{cases}
d_g(\bm{p}, w), & \text{if } \exists \, \bm{q}_k \text{ such that } l_i < P_i(\bm{q}_k) < r_i, \\
& \forall k = 0, \dots, 26, \\
\frac{w}{2}, & \text{otherwise}.
\end{cases}
\label{eq:distance}
\end{equation}
where,
\begin{equation}
d_g(\bm{p}, w) = f(\bm{p}) \ + \min_{\substack{k=0 \\ \exists \, \bm{q}_k, \ l_i < P_i(\bm{q}_k) < r_i}}^{26} d_{\bm{q}_k}\left(\frac{1}{w}(\bm{p} + \bm{h}(\bm{p}))\right) \,, \label{eq:pameso-sdf}
\end{equation}



In this condition, the terms \( l_i \) and \( r_i \) represent the minimum and maximum bounds of the corresponding polynomial values \(P_i(\bm{q_k})\) when the \( i \)-th polynomial is evaluated with the point \(\bm{q_k}\). The interval length \( (l_i,r_i) \) controls the width (or thickness) of the macroscopic object. In some cases, it may be necessary to use $R$ instead of $P$. These polynomials can be used to create the macro-shape of the object based on the roots of the polynomials; basically, the particle jittering follows these polynomial functions.  When the roots of these polynomials are true, the microgeometry on the surface can be generated using the SDF \( d_g(\bm{p}, w) \).

For instance, the following polynomial can be used to generate the macrosurface with microstructure, as shown in Figure 10 in the supplemental material.
\begin{align}
P(q) &= 2q_x + q_y^2 + q_z^2 - q_x q_y - q_y q_z - q_z q_x \,.
\end{align}



\begin{figure}
    \centering
    %\includegraphics[width=0.33\linewidth]{images/cheese_tightly_loose.png}&
   \begin{tabular}{@{}c@{}c@{}}
    \includegraphics[width=0.5\linewidth]{images/fibers_primitive1.png}
    \includegraphics[width=0.5\linewidth]{images/fibers_primitive.png}
    %\includegraphics[width=0.33333\linewidth]{images/gyroid_1-25.png}
    \end{tabular}
  \caption{ Fibrous microstructure generated from directly using cylindrical primitive, each fiber is of diameter 0.028 mm}
  \label{fig:primitive-fibers}
\end{figure}


\subsection{Modeling Granular Media with Particle Piling}\label{sec:pp}

After modeling particle suspensions and particle agglomerations, we focus on particle piling, where particles are settled in a contact position and can not merge or intersect. We use the same regular lattice of spherical particles used for the particle agglomeration, which is basically based 27-neighborhood of the point $\bm{p}$. Like traditional finite element methods, we don't need to find the collisions between particles(or grains). We consider rock piles and sand as interesting case studies for piling structures. We place spherical particles in a cubic regular lattice with the maximum possible size, and we do grid deformation or particle deformation to generate piling structures. Here, no union and intersection operations on particle clouds are allowed because every grid cell already contains a particle. Only one rotation operation with respect to the coordinates systems x, y, and z is allowed.

The SDF equation \ref{eq:pa-sdf} for the particle agglomeration can be changed in the following manner for the generation of particle piling
\begin{equation}
d_g(\bm{p}, w) = f(\bm{p}) + \min_{i=0,\dots,26} d_{\bm{q}_i}\left(\frac{1}{w}((\bm{R_{ \theta}}\bm{p}) + \bm{P}(\bm{p})\bm{N}(\bm{p}))\right) \,, \label{eq:pp-sdf}
\end{equation}

In the above equation, the term $\bm{R_{ \theta}}$ refers to the rotation matrix with angle  $\theta = P$, where we consider even angle for the rotation is also a polynomial in $\bm{p}$. The term $\bm{P}(\bm{p})\bm{N}(\bm{p}))$ generates the grid deformation using a product of the polynomial function $ P(p)$ and the noise function $N(p)$. For instance, sparse convolution noise \cite{frisvad2007fast} is used as $N(p)$ and $\theta$ as the gyroid function in $\bm{p}$ to generate patterns similar to the rock piles in Fig.\ref{fig:svbunny}. The term $ P(p)$ in the above equation controls the degree of convexity to the concavity of the grains in the same particle cloud, where the smooth transition between convexity to concavity is in the same cloud.

